On Affine Reachability Problems

We analyze affine reachability problems in dimensions 1 and 2. We show that the reachability problem for 1-register machines over the integers with affine updates is PSPACE-hard, hence PSPACE-complete, strengthening a result by Finkel et al. that required polynomial updates. Building on recent results on two-dimensional integer matrices, we prove NP-completeness of the mortality problem for 2-dimensional integer matrices with determinants +1 and 0. Motivated by tight connections with 1-dimensional affine reachability problems without control states, we also study the complexity of a number of reachability problems in finitely generated semigroups of 2-dimensional upper-triangular integer matrices.

==> cc-by <==
%PDF-1.3
%âãÏÓ
1 0 obj
<</Metadata 2 0 R/Pages 3 0 R/Type/Catalog>>
endobj
2 0 obj
<</Length 14818/Subtype/XML/Type/Metadata>>stream
<?xpacket begin="" id="W5M0MpCehiHzreSzNTczkc9d"?>
<x:xmpmeta xmlns:x="adobe:ns:meta/" x:xmptk="Adobe XMP Core 5.0-c060 61.134777, 2010/02/12-17:32:00        ">
   <rdf:RDF xmlns:rdf="http://www.w3.org/1999/02/22-rdf-syntax-ns#">
      <rdf:Description rdf:about=""
            xmlns:xmp="http://ns.adobe.com/xap/1.0/"
            xmlns:xmpGImg="http://ns.adobe.com/xap/1.0/g/img/">
         <xmp:CreatorTool>Adobe Illustrator CS5</xmp:CreatorTool>
         <xmp:CreateDate>2012-09-19T10:17:41+02:00</xmp:CreateDate>
         <xmp:ModifyDate>2012-09-19T10:17:41+02:00</xmp:ModifyDate>
         <xmp:MetadataDate>2012-09-19T10:17:41+02:00</xmp:MetadataDate>
         <xmp:Thumbnails>
            <rdf:Alt>
               <rdf:li rdf:parseType="Resource">
                  <xmpGImg:width>256</xmpGImg:width>
                  <xmpGImg:height>92</xmpGImg:height>
                  <xmpGImg:format>JPEG</xmpGImg:format>
                  <xmpGImg:image>/9j/4AAQSkZJRgABAgEASABIAAD/7QAsUGhvdG9zaG9wIDMuMAA4QklNA+0AAAAAABAASAAAAAEA&#xA;AQBIAAAAAQAB/+4ADkFkb2JlAGTAAAAAAf/bAIQABgQEBAUEBgUFBgkGBQYJCwgGBggLDAoKCwoK&#xA;DBAMDAwMDAwQDA4PEA8ODBMTFBQTExwbGxscHx8fHx8fHx8fHwEHBwcNDA0YEBAYGhURFRofHx8f&#xA;Hx8fHx8fHx8fHx8fHx8fHx8fHx8fHx8fHx8fHx8fHx8fHx8fHx8fHx8fHx8f/8AAEQgAXAEAAwER&#xA;AAIRAQMRAf/EAaIAAAAHAQEBAQEAAAAAAAAAAAQFAwIGAQAHCAkKCwEAAgIDAQEBAQEAAAAAAAAA&#xA;AQACAwQFBgcICQoLEAACAQMDAgQCBgcDBAIGAnMBAgMRBAAFIRIxQVEGE2EicYEUMpGhBxWxQiPB&#xA;UtHhMxZi8CRygvElQzRTkqKyY3PCNUQnk6OzNhdUZHTD0uIIJoMJChgZhJRFRqS0VtNVKBry4/PE&#xA;1OT0ZXWFlaW1xdXl9WZ2hpamtsbW5vY3R1dnd4eXp7fH1+f3OEhYaHiImKi4yNjo+Ck5SVlpeYmZ&#xA;qbnJ2en5KjpKWmp6ipqqusra6voRAAICAQIDBQUEBQYECAMDbQEAAhEDBCESMUEFURNhIgZxgZEy&#xA;obHwFMHR4SNCFVJicvEzJDRDghaSUyWiY7LCB3PSNeJEgxdUkwgJChgZJjZFGidkdFU38qOzwygp&#xA;0+PzhJSktMTU5PRldYWVpbXF1eX1RlZmdoaWprbG1ub2R1dnd4eXp7fH1+f3OEhYaHiImKi4yNjo&#xA;+DlJWWl5iZmpucnZ6fkqOkpaanqKmqq6ytrq+v/aAAwDAQACEQMRAD8AjfkryVpn5jaZN5z85zXG&#xA;qaxqlxMxLTOiRIjlFjjVCKKKbDoBQAYCWJLIf+VDflp/1b5f+kib/mrBaLd/yob8tP8Aq3y/9JE3&#xA;/NWNrbv+VDflp/1b5f8ApIm/5qxtbd/yob8tP+rfL/0kTf8ANWNrbv8AlQ35af8AVvl/6SJv+asb&#xA;W3f8qG/LT/q3y/8ASRN/zVja27/lQ35af9W+X/pIm/5qxtbd/wAqG/LT/q3y/wDSRN/zVja27/lQ&#xA;35af9W+X/pIm/wCasbW3f8qG/LT/AKt8v/SRN/zVja27/lQ35af9W+X/AKSJv+asbW3f8qG/LT/q&#xA;3y/9JE3/ADVja27/AJUN+Wn/AFb5f+kib/mrG1t3/Khvy0/6t8v/AEkTf81Y2tu/5UN+Wn/Vvl/6&#xA;SJv+asbW3f8AKhvy0/6t8v8A0kTf81Y2tu/5UN+Wn/Vvl/6SJv8AmrG1t3/Khvy0/wCrfL/0kTf8&#xA;1Y2tqF3+Sn5T2cfq3dv9Xi/nlu5UXb3Zxja2UCn5Y/kY7BUuLZmPRRqJJP8AyUxtNlNF/Ij8smUM&#xA;thIysKgi5mIIP+yxtFt/8qG/LT/q3y/9JE3/ADVja27/AJUN+Wn/AFb5f+kib/mrG1t3/Khvy0/6&#xA;t8v/AEkTf81Y2tu/5UN+Wn/Vvl/6SJv+asbW3f8AKhvy0/6t8v8A0kTf81Y2tu/5UN+Wn/Vvl/6S&#xA;Jv8AmrG1t3/Khvy0/wCrfL/0kTf81Y2tu/5UN+Wn/Vvl/wCkib/mrG1t3/Khvy0/6t8v/SRN/wA1&#xA;Y2tse86+StM/LnTIfOfkya40vWNLuIWBWZ3SVHcI0ciuTVTXcdCKgjCCkFkP5Df+S00//jLcf8nm&#xA;wFBeg4oWzTRQxPNM6xxRqWkkchVVQKkknYAYq8Z88f8AOQ9paSyWXlWBLyVaq2ozg+iD0/dICrP/&#xA;AKxIHsRhpkIvMz5v/NjzfdtBZ3Wp6hMetnpqSUoeg9K2Ar7VGGk0jf8AlW357+n6n6A8wcacqejd&#xA;cqUr9nrX2xSg/wDF/wCbPlG7WG9u9U0+ZelpqSSEbHceldKafQMaRT0ryT/zkTaXUsdl5qt1s5Go&#xA;q6jbgmGv/FkZ5Mn+spI9gMFIMXs0E8M8KTwSLLDKoeOVCGVlYVDKw2IIwMV+KuxV2KuxV2KuxV2K&#xA;uxV3TFXiH5ifnjeyX58v+SQZrhn9B9QjT1XeQnj6dslDy32D71/ZHQ4QGQCt5Z/5xP8AzW828dV8&#xA;1aimj+uOR+vM93e0O4LRg0X5NICPDCyZPcf84NTrCxt/OayTAfAkmnFFJ92Fy5H/AAJxV595k/Lb&#xA;87fycP6RhlM+hq3x3lkzXFnuek8LqDHX+ZkpU7NXFaej/ll+aum+crZreZVs9cgXlNaA/DIo6yQ1&#xA;3K+I6j8ciQwIZ5ih2KuxV2KuxV2KuxV2KvPvz5/8lpqH/GW3/wCTy4hId+Q3/ktNP/4y3H/J5sSp&#xA;eg9MUPmr84/zXn8wXkuhaPLx0G3fjLKh/wB6pFPUkf7rU/ZHf7XhQgMwHpv5H/8AOKC31tb+Y/zB&#xA;jdLeUCWz0AExuykVV7plIZa/77Wh/mI+zhS+ptI0TR9GsY7DSLKDT7KIUjt7aNYox/sUAGKo3FUJ&#xA;quj6TrFjJYatZQX9lL/eW1zGk0bfNHBGKvl787f+cTIoLafzB+XcTn0+Ul35eJLkr1LWjN8RI/30&#xA;a1/ZPRcVeTfk9+alx5bv49G1aYtoFw/EM+/1WRj9ta9Iyftj6R3qCEEPpoEMAymoO4I6EYGDsVdi&#xA;rsVdirsVdirsVeU/n/53m0bQotCsZDHe6sG+sOuxS1XZh/z0J4/LliGQD0T/AJxh/I2y8s6Fbeb9&#xA;dtlk8y6nGJbNJVBNlbSCqBQeksimrHqB8O3xVkye2eZIdWm8u6pDo0gh1eSznTTZW2VLlomELH2D&#xA;0OKvkT/nHLyV+b+m/nFHeahp+p6fZR+ufMNxfLLHFMrRMFDPJ8MztKystCf5umKvsmeCC4gkgnjW&#xA;WCVSksTgMjowoysp2II2IOKvij/nIf8AKqf8r/N9j5v8p1tdFvpy1uqfZtLwAu0HvHIoYovhyXoN&#xA;1XrHlHzHb+Y/LdhrUA4rdxBnj68JFJWRP9i6kZFrKb4q7FXYq7FXYq7FXYq8+/Pn/wAlpqH/ABlt&#xA;/wDk8uISHfkN/wCS00//AIy3H/J5sSpUvz083SaD5Oa0tn4X2sMbaNgaMsQFZnH+xIX/AGWIUBj3&#xA;/OJf5R2/mbX5vN+swCbRtDkCWULiqTX9A4LDusCkNT+Yr2BGSZvtLFUHbazo91cNb2t9bz3CV5Qx&#xA;So7inWqqScVRmKoW91bSrAqL69gtS/2BPKkZb5ciK4qiUdJEDxsHRhVWU1BHiCMVfG3/ADl3+U1r&#xA;oGtW/nXSIRFp2tSmLUoUFFjveJcSCn+/1Vif8pSf2sVTb8h/NsmueTvqNy/O90ZhbMxNWaBhWBj9&#xA;AKf7HIlgQ9JxQ7FXYq7FXYq7FXYq+ffNNgnmv/nIzTNBuR6tl9csLOVDuDbgJNOtD/rvhDMPu0AA&#xA;UGwHQYUvmL/nNzWdWs7LyjZWl5Nb2l09/LcwxOUWR4BbiItSleAlenzxV8p/pbVf+Wyf/kY/9cVf&#xA;ol+SWpX+p/lP5XvtQuHuryaxQzXEpLO5UlQWY7k0HU4qlv8AzkboNvrP5NeZI5lBeygF/A56q9qw&#xA;kqPmgZfpxV4F/wA4238k3lHULNyStrelo69AssaniP8AZKT9OAsZPW8DF2KuxV2KuxV2KuxV59+f&#xA;P/ktNQ/4y2//ACeXEJDvyG/8lpp//GW4/wCTzYlS8y/5yR1F5vN9hY1/dWlkHp/lzSNy/wCFRcIT&#xA;F9a/84+eXodC/J3yzBGoD3louozMOrPe/wCkAn5I6r8hhZPnH/nJv83/ADJ5h87XfkbRbiSHRNNm&#xA;FlLb27FWvLvYSCXj9pUk+BU6VFfkqp63/wA4g/mJovlf9O2V/Df6zbIJ5tHs1k9YU3IglH95Iv8A&#xA;KFFf2amlVWd6t+ZP5v8A5Z/kZEPNxj/xbqFz9S0K4lkE91FbGMu8t1TkjSRgUT4iasvMbGqryr8r&#xA;vyH85/m7b3/ma81kWtuJzCb+99S5nuJwAz0BYHivIVYt12HfFXpH5E/lz+fPkX8xp9L4f86hbzel&#xA;qkk8rCxniYBhNZqw5mSjVBVevwuRir2b/nIDQIdb/J3zRbyKC1rZPfxN3V7L/SKj5iMj5HFXyR/z&#xA;jdqDw+b7+xqfSurJnIHTnDInEn/Yu2AsZPo7AxdirsVdirsVdirsVfP/AJgvo/K3/OSWma1dfu7L&#xA;69YXMjntA6pDM+/hxc4QzD7rwpeGf85W/ljP5s8qQeYY9QW0Tyla393JbtGXM4lWFuKsGXhT6v4H&#xA;rir438m+XH8zea9J8vRzi1fVbqK0W4ZeYQysF5FQVrSvjir9Gfy88qSeUvJWkeW5LkXb6XbiBrlV&#xA;MYcgk1CktTr44qxv/nIfWbfSfya8zzTEVubX6lEp6s906wgD5By30Yq+ff8AnGyyli8qaldsCEub&#xA;3jHXuIo1qR9L0+jAWMnruBi7FXYq7FXYq7FXYq8+/Pn/AMlpqH/GW3/5PLiEh35Df+S00/8A4y3H&#xA;/J5sSpeSf85CwvH+YRduk1nA6/IFk/WpwhlF9wflbeRXv5aeVLqL7MukWJp1oRboGX6CKYUvhv8A&#xA;MAyeWf8AnILV73Uo2RLTzG2pOgHxGCS7+toR/rROCMVfcutfmR5K0jyk/mu51W3k0YQmaCaGRGM/&#xA;w8ljhHIc5GqAF998VfNn/OUXnHy35/8AIPlvzL5XvBeWFhey21/GVKTW8t1CHjWaM7rX0GFfsnsT&#xA;irO/+cPvN2hXP5bNoH1mGLVtMurh5rVmCyvDKRKs1CfiXcqT2479sVegWX56/lleedpvJsWrxjV4&#xA;5I4YXNDbXE0gH7mGdSyM6khSpp8Wwqa4qm/5oXcdp+Wvmu5k+zFpF81OlT9Weg+k7Yq+H/8AnHmF&#xA;pPzCDjpDZzu3yJRP1tgKJPpzAwdirsVdirsVdirsVeSf85BeSJtW0aDzBYxGS70pWW6VRVmtWPIt&#xA;/wA8m3+RJ7YhkC9T/wCcZvzusvNvl638r6xcLH5p0qJYovUahvLeNaLIhP2pEUUkHX9rxpJkz786&#xA;/wDyUfm//tlXX/Jo4q+FfyU/8m55Q/7atr/ydGKv0dkkjijaSRgkaAs7sQFVQKkknoBir4u/5yR/&#xA;NpvzG8zWXkrymTeaRY3FFliNVvL1hw5p/wAVxBmVW6GrN9mhxV6d5L8tQeWvLFho0RDG1j/fSD9u&#xA;Vzzkb6XY09siwKdYodirsVdirsVdirsVeffnz/5LTUP+Mtv/AMnlxCQ78hv/ACWmn/8AGW4/5PNi&#xA;VLDP+cl9BcnSNfjWqAPY3L+G5lh/5mYQmL2n/nELz1Brf5cny5NIP0l5claPgT8TWs7NJC/+xYun&#xA;tQeOFkyD85v+ce/LX5lNHqH1htJ8wwoIk1GNBIskY3CTxVTnSvwsGBHuNsVeNWP/ADhB5ha943/m&#xA;e0jsQR+8gglklI7/AAOY1H/BHFX0Dov5K+QNK/L6byIlh9Y0W7BN88xBnnmNP37yKF/eAqpUqBxo&#xA;KYq8F1z/AJwh1QXrHQfMsD2LN8CX0LpKiE9C0XNXI8eK19sVej/k3/zjB5f8hammvape/pvXogfq&#xA;j+n6VvbFhQsiFnZnpUB2O3YV3xVT/wCcuvO8Gh/lk2hRygaj5jlW3jjB+IW0LLLO/wAtlj/2WKvE&#xA;P+caNCfnrGuyJRKJZW7+Jr6sw+ikeAsZPdcDF2KuxV2KuxV2KuxVxAYFWFQdiD0IxV4Z+YX5J6pZ&#xA;akfMXkYtFIj+udPhYxSwyKeXO1YEd9+HUfs16AgsgUw8r/8AOXX5g+X4v0R5x0eLXBCPTkaflZXl&#xA;OlJTwdG28YgT3JwsmSTf85oeXIohJZeR/wDSxuvO5iRVauxDLAzdN+g/jirz7zX+b35y/nAz6Np9&#xA;ubXRnPGaw08NHCy7EfWrhz8XyLBT/Lits/8Ayv8Ayk0/yfF9evGW816VSr3Ar6cKt1SIHx7uRU+w&#xA;yJLAl6Dih2KuxV2KuxV2KuxV2KvPvz5/8lpqH/GW3/5PLiEhL/yS8w6BZfl3YW95qdpbTrJcFoZp&#xA;443AMzEVVmB3xKlmOv6boPnTy1faWl1DdW86lBcQOsoimWjI1UPVWoaV3HzxV83+U/M3mv8AKT8w&#xA;xeRx8L2wcwX9mxIjubZyCyE/yuoDI1NjRu2SZvvfyD+YHlrz15eg1vQbgSwyAC4t2IE1vL+1FMgJ&#xA;4sPuPUVGKskxV2KuxVj/AJ58+eWvJGgTa35guhb2sdRFEKGWeShKxQptydqfIdTQb4q+BvPPnHzT&#xA;+bf5g/W2iJnu3FtpWnqSUt7dSSqV9hV5H8anYbBV9GeXNK0PyT5XsdLlu4baGEcZLmd1iEs71aRq&#xA;uRuxrQdh8siwRn+LvKn/AFerD/pJh/5qxRTv8XeVP+r1Yf8ASTD/AM1YrTv8XeVP+r1Yf9JMP/NW&#xA;K07/ABd5U/6vVh/0kw/81YrTv8XeVP8Aq9WH/STD/wA1YrTv8XeVP+r1Yf8ASTD/AM1YrTv8XeVP&#xA;+r1Yf9JMP/NWK07/ABd5U/6vVh/0kw/81YrTv8XeVP8Aq9WH/STD/wA1YrSE1HVfy91JAmo3mkXq&#xA;DotxJbSgfQ5bFKVw6Z+TUMhkjh0AOTWp+qGh67VrT6MV3TyHzP5OgiWGDVtOiiQUSNLiBVA9gGpi&#xA;q/8Axd5U/wCr1Yf9JMP/ADViinf4u8qf9Xqw/wCkmH/mrFad/i7yp/1erD/pJh/5qxWnf4u8qf8A&#xA;V6sP+kmH/mrFad/i7yp/1erD/pJh/wCasVp3+LvKn/V6sP8ApJh/5qxWnf4u8qf9Xqw/6SYf+asV&#xA;p3+LvKn/AFerD/pJh/5qxWnf4u8qf9Xqw/6SYf8AmrFaYJ+dvmHQL38u7+3s9TtLmdpLcrDDPHI5&#xA;AmUmiqxO2ISHzPkmbO/yk/MRvJ+vEXTM2i3/ABjvkFTwI+xMoHdK706j3pgKCHun5g/l3ofn7SIb&#xA;y2nSPUEj5adqUZDI6N8QR+P2oz2p06juCGINPBLK/wDzH/KnzN69pLPo+oLtyX47e5jB7g1jmT59&#xA;PY5Jm978pf8AObdt6KRebvL8izCnO80p1ZW/6N52Xj/yNOKs1/6HD/J/0PUrqXP/AHx9VHPrTr6n&#xA;D3+1irC/Nv8Azm3ZiB4vKXl+Rp2BEd3qjqiqfEwQM/L/AJGjFXgeo6p+ZH5r+ZhNeTT6xqB2WtEt&#xA;7aNj0UCkcKbfT7nFXvH5eflxovkLSZr69mjk1Noy9/qT/CkcY+IpGW+ygpuf2u/YCNsCbeGfmz+Y&#xA;b+cNf/0YsujWPKOwjO3Op+OZh4vTbwFO9cIZAMGwpdirsVdirsVdirsVdiqM0jSNR1jVLXStNhNz&#xA;qF7KsFrApALyOaKoLEDc+JxVnx/5xv8AztAJPlaeg32ltifuEuKpFpf5UfmJqkGrTWOhzy/oJmTV&#xA;4SUSe3ZFLkPA7LL9kGlF37YqgvJ/kHzh5yu57TyzpkupT2sYluFjKKEQtxBLSMi7noK1+44qkdxB&#xA;Lb3EtvKAJYXaOQAhgGU0NGUlTuOoOKqeKuxV2KuxV2KuxV2KuxV2KuxV2KvQfy0/N7VfKDCxuVa+&#xA;0JmJa1r+8iLdWhJ29yp2Psd8BCCH0HputeR/PeklIWttVtSA0tnMqmSM9KtE/wASHfZvuOBixLWP&#xA;+cdvI945ksZbrTWP+643EsQ+iUM//D42vEkv/QslhX/jvy0/5hl/6qYbTxJ1o/8Azjt5Hs3El9Ld&#xA;akw/3XI4iiP0RBX/AOHwWjiZZqWteRvIWkhJWttLtlFYrOBVEsh6VWNficnux+k4rzfPv5l/m7q3&#xA;m92sbZWsdCVqra1/eSlT8LTMPDqFGw9zvhAZAPPsKXYq7FXYq7FXYq7FXYq7FWa/kp/5Nzyh/wBt&#xA;W1/5OjFX1Xqo0GD/AJyEa6n/ADRuNOu2ntFPkjjPHAzNaxJHCZWl+rsJqh+Pp1q382+KvM9Z/MzX&#xA;/wAu/wDnKLV9V1y2FlpWrvbwanbRP6sbWPpJFDdKQBVk9P1D8NftL3rirL/znvvK/wCTPkTVdN8n&#xA;J9W1rz5dTTCZD/c25A9Uxsv2URZOMQHQuSOmKvjzFXYq7FXYq7FXYq7FXYq7FXYq7FXYq7FVW2ur&#xA;m1nS4tZngnjNY5YmKOp8Qy0IxVm+kfnd+Y2mosf6SF7EvRbuNZT9MlFkP0tgpFJz/wBDIee/T4fV&#xA;NN5Up6nozcvn/fU/DGl4Ul1b87fzG1JGj/SQs4mrVbSNIj9ElDIPobGlphNzdXN1O9xdTPPPIayS&#xA;ysXdj4lmqThSpYq7FXYq7FXYq7FXYq7FXYq7FWQfl/5itfLXnfQ9fu4nmttLvYbqaKKnNlicMQvI&#xA;gV27nFXuWs/nr/zj3qfmw+crryNqV35nEsM63ctwUQyWypHExjW4aL4FjX/dfb6cVeO/mt+Y+ofm&#xA;H5xufMd5brZh0SC1s0YuIoYgeKlyByNSSTQbnpirKfz6/N/RPzG/w5+i7K5s/wBDW8sE/wBa9P42&#xA;k9OhTgz7fuz1xV5NirsVdirsVdirsVdirsVdirsVfTNx/wBCS/WJf97Ptt/d/pPh1/Z9vDFVP/rC&#xA;X/l+/wC5nirv+sJf+X7/ALmeKu/6wl/5fv8AuZ4q7/rCX/l+/wC5nirv+sJf+X7/ALmeKu/6wl/5&#xA;fv8AuZ4q7/rCX/l+/wC5nirv+sJf+X7/ALmeKu/6wl/5fv8AuZ4q7/rCX/l+/wC5nirv+sJf+X7/&#xA;ALmeKu/6wl/5fv8AuZ4q7/rCX/l+/wC5nirv+sJf+X7/ALmeKu/6wl/5fv8AuZ4q7/rCX/l+/wC5&#xA;nirv+sJf+X7/ALmeKu/6wl/5fv8AuZ4q7/rCX/l+/wC5nirv+sJf+X7/ALmeKu/6wl/5fv8AuZ4q&#xA;7/rCX/l+/wC5nirv+sJf+X7/ALmeKu/6wl/5fv8AuZ4q7/rCX/l+/wC5nirv+sJf+X7/ALmeKu/6&#xA;wl/5fv8AuZ4q7/rCX/l+/wC5nirv+sJf+X7/ALmeKu/6wl/5fv8AuZ4qqW//AEJL9Yi/3s+2v95+&#xA;k+HX9r28cVf/2Q==</xmpGImg:image>
               </rdf:li>
            </rdf:Alt>
         </xmp:Thumbnails>
      </rdf:Description>
      <rdf:Description rdf:about=""
            xmlns:xmpTPg="http://ns.adobe.com/xap/1.0/t/pg/"
            xmlns:stDim="http://ns.adobe.com/xap/1.0/sType/Dimensions#"
            xmlns:xmpG="http://ns.adobe.com/xap/1.0/g/">
         <xmpTPg:NPages>1</xmpTPg:NPages>
         <xmpTPg:HasVisibleTransparency>False</xmpTPg:HasVisibleTransparency>
         <xmpTPg:HasVisibleOverprint>False</xmpTPg:HasVisibleOverprint>
         <xmpTPg:MaxPageSize rdf:parseType="Resource">
            <stDim:w>31.044444</stDim:w>
            <stDim:h>10.936111</stDim:h>
            <stDim:unit>Millimeters</stDim:unit>
         </xmpTPg:MaxPageSize>
         <xmpTPg:PlateNames>
            <rdf:Seq>
               <rdf:li>Cyan</rdf:li>
               <rdf:li>Magenta</rdf:li>
               <rdf:li>Yellow</rdf:li>
               <rdf:li>Black</rdf:li>
            </rdf:Seq>
         </xmpTPg:PlateNames>
         <xmpTPg:SwatchGroups>
            <rdf:Seq>
               <rdf:li rdf:parseType="Resource">
                  <xmpG:groupName>Standard-Farbfeldgruppe</xmpG:groupName>
                  <xmpG:groupType>0</xmpG:groupType>
               </rdf:li>
            </rdf:Seq>
         </xmpTPg:SwatchGroups>
      </rdf:Description>
      <rdf:Description rdf:about=""
            xmlns:dc="http://purl.org/dc/elements/1.1/">
         <dc:format>application/pdf</dc:format>
         <dc:title>
            <rdf:Alt>
               <rdf:li xml:lang="x-default">CC-BY_icon</rdf:li>
            </rdf:Alt>
         </dc:title>
      </rdf:Description>
      <rdf:Description rdf:about=""
            xmlns:xmpMM="http://ns.adobe.com/xap/1.0/mm/">
         <xmpMM:RenditionClass>proof:pdf</xmpMM:RenditionClass>
         <xmpMM:DocumentID>uuid:ebb30592-243e-eb4a-9564-284441576148</xmpMM:DocumentID>
         <xmpMM:InstanceID>uuid:9ac8f4ed-f591-f049-aee8-305fac061b6c</xmpMM:InstanceID>
      </rdf:Description>
      <rdf:Description rdf:about=""
            xmlns:pdf="http://ns.adobe.com/pdf/1.3/">
         <pdf:Producer>Adobe PDF library 9.90</pdf:Producer>
      </rdf:Description>
   </rdf:RDF>
</x:xmpmeta>
                                                                                                    
                                                                                                    
                                                                                                    
                                                                                                    
                                                                                                    
                                                                                                    
                                                                                                    
                                                                                                    
                                                                                                    
                                                                                                    
                                                                                                    
                                                                                                    
                                                                                                    
                                                                                                    
                                                                                                    
                                                                                                    
                                                                                                    
                                                                                                    
                                                                                                    
                                                                                                    
                           
<?xpacket end="w"?>
endstream
endobj
3 0 obj
<</Count 1/Kids[5 0 R]/Type/Pages>>
endobj
5 0 obj
<</ArtBox[0.0 0.0 88.0 31.0]/BleedBox[0.0 0.0 88.0 31.0]/Contents 6 0 R/LastModified(D:20120919101741+02'00')/MediaBox[0.0 0.0 88.0 31.0]/Parent 3 0 R/PieceInfo<</Illustrator 7 0 R>>/Resources<</ExtGState<</GS0 8 0 R>>/Properties<</MC0<</Color[20224 32768 65535]/Dimmed false/Editable true/Preview true/Printed true/Title(svg2759)/Visible true>>>>>>/Thumb 9 0 R/TrimBox[0.0 0.0 88.0 31.0]/Type/Page>>
endobj
6 0 obj
<</Filter/FlateDecode/Length 2006>>stream
H‰|W»®Ý6ìõú#"Ëw'HAŠÔÁc×ìTùûÌ̒'nl¸‡#ñ±Ü]½ùåÞÙß¼{ö~|»oŸ·°§¸÷¾?ðóåýöûþ׎Zێÿ£óËۛŸû‡¿·Ï{ÜþânG
Öö")VÊþü´ñù§­§#ZÝሹï/[χõ¶p/G²'}ƒåvä÷çl–`^§ŒµxFÿÆÞÆ
Glžø3ð8èï¹ý¹ýºù¸G͘…=­Ä›Ýùh!cø";'aˆA
¶çÐoh"áæ
[<B6¬³|ô:î쨼_9NŒV¶£ìHGÖl‡Øï(õ"ôZõ¥ÝàìP¯"ž›lH·"Ö·íŽó¼£9³®z´<vÝ_£¹jLø £HÊçݶqôÖ¸t>`¨ºBÁ˜>¦—­ÕÊw3°Äpy=b/çÀTìÜmÁyÚs[Öu'v[—˜æ-^ÝÕ9I'ל(ùl¶£5œw'¤'`•6	'ÃAÁ»O¼OClÖá¤
®ø_
-ˆ`-gUq>v.¯s-3ǚqn²¡Y2ç´Áÿ%Ös\³ïä¨]‰,µxR!Átgåԁ˜wô§aœ´oÐ
Ž˜ë"/'ÿI"Piײ»ÁúD؁2<ٝ\vXôSî!Y =ƒ¬ÍåÖâpÔêÑöªùZ;Rqû!I	Á"Cð,ÉxªVŒcðY68KVC88lr3´c÷i€.$DOŠÀ€˜]ŽÊ§/ž¾ðÓA#'$Ê	8b"Ç"\ A£ûÑ]æÌP"Jûzg(¢ž7\ñ¹Áû H'Øf¼É–ÊH2öˆX4©Èî•¢+9ð1˜5ÇA‰«œ:äJ±6óR'˜ˆ+<rˆŠ§7B-q§,cdwM§êµÎI1ka)û5.Ý·r"p*ÆJÊ(
¶(1!nº¤Êt@
OÒn)éM	¾]lJúçÑTåµ?'nQšV)ÝRÕ«ž8OUÂÁ"ÅÃb]øea+£N±¸i$*à}…ŸÆ­px@™7ðxªªB‰Pß=¡2Ø_甎<x €Ñ.ˆºÑY+éÕôDZôü
ƒPbeeö¼R­@í/¡ÎÝr£ÓÛPØqŒ'&ì¢>æÅâOèÞÈEËÛD«¨Ê39Œ'Á3~7×AÑÕø:†Gó7²ˆîa_Ûü^ÕæQ•×àK»]–¼'ÎU"™M¢1¼0яÀÃ=l½ƒçC—:ö˜õ~lj½/™ë³XëÚt"Uâr{K~gm˜lñ
Z9s¦°"œp÷Ëæµ^‰üÁõ¸M–ý¬žlŒÉ \NŒ³¬)°Lp ®R
ögw3µƒA˜È%Ó¡•_µäs»÷jÁ+Rõžµ¾w¹"ò")ûÉS¨#¹z¡7Ë¡M"û©
I@"›DÕ¥J¦=d"ª¦¢× ¬}E}P¿'×qËKp8º'çà
ÞÄ3x¾n…G{^±kHø+v'WVì€2› <¤CPÃ3£Üèæ¾êŠ6Ô!!ù¾¦àÄÌÀxFéPÒ-z÷(ñ_ŒròßDgø&žáãRUyÅ/ºjž*´3€0¨ÖÀŽ"âÀŠR4æôQÝ#ÈÛ·W!ÄaÔ)*5ˆ#»YÖ±J£q·DõΨmÉj±`6œ+#Oècè…TohªÛMƒø"DŠ<VåüAÚL¨<ISzÊÌÆ$‡Wc­kEh‰r"BË•Hӌ8?Á²×!+2‹sb%nªé-J¿ú$~"yžþ	Bˆv?§e¤q®œ–5ô=XçÕO—Ò@vsMýݧ
ŸJÈrä+|…ô	¬õdžOJLÉû6Þ8xÿà'·äëðL]Ö}ZEnB¥_híz·š|9ÃYÐ%«6‹Š¡ce
%*ɛµqÁ‹Èþ	So.FºÔ|îíŽà\Üö¡ŒäÇð([\fO¤®®•Ùää¹ìîÚï€6àçÆî¬_‡ÎÅZ¯9p"š¼úÜ&Œì†I(ê
nÕù™pŽ¤¿·7T'ˆ¹jÁµçÂ~àcZñ¿Ÿº¥£óE‡nê?¯þ`÷–¥3¯²<&iÁڄ/²ÔÖ[
©6™`–žiaÐ'2<|á8Ö?7ÛWpÍ×ð«V¡‰")0¼…ûÍÐ4NA€UTKª°OkÞE:ìE…‡]ŽùwÜ(Ÿo/¯Ö<þ³áãÕieÙ׆'æn%Só½‰dÏfûÏ=¤J#ʆ ¾¶zòH.¹^ªNû¸)K8kHÔ)kXÁf:²¼r7Oxnzê²+Eúh"(­1‹£>Òí†rÕˆ~æëÌÕmÖ©'†uf)*ªÃË0ËæBËօ‹¾
¸´‹.¹zçâuÜoσ«-×<–ÃÜˏõi[ø¹Ê¨µæˆÄmÌþUÔÕ³0O©ÚTÔ+iݽF·ÞOpš:1¤8g¹0ò{hœûRªJœ‰mCN›=Eš‰^(£ní'O~8Ø	™ØŠ†BQU©µs'°Ô%££ªŠð;qLɞ—1Ûi.­( ,v´|ù€þéÓ?,Ÿ6ývó¨³ø§wowüü+ÀÞÑæ
endstream
endobj
9 0 obj
<</BitsPerComponent 8/ColorSpace 10 0 R/Filter[/ASCII85Decode/FlateDecode]/Height 3/Length 27/Width 11>>stream
8;Ue`5QQie@L]UK5_&k8&ao`Q~>
endstream
endobj
10 0 obj
[/Indexed/DeviceRGB 255 11 0 R]
endobj
11 0 obj
<</Filter[/ASCII85Decode/FlateDecode]/Length 428>>stream
8;X]O>EqN@%''O_@%e@?J;%+8(9e>X=MR6S?i^YgA3=].HDXF.R$lIL@"pJ+EP(%0
b]6ajmNZn*!='OQZeQ^Y*,=]?C.B+\Ulg9dhD*"iC[;*=3`oP1[!S^)?1)IZ4dup`
E1r!/,*0[*9.aFIR2&b-C#s<Xl5FH@[<=!#6V)uDBXnIr.F>oRZ7Dl%MLY\.?d>Mn
6%Q2oYfNRF$$+ON<+]RUJmC0I<jlL.oXisZ;SYU[/7#<&37rclQKqeJe#,UF7Rgb1
VNWFKf>nDZ4OTs0S!saG>GGKUlQ*Q?45:CI&4J'_2j<etJICj7e7nPMb=O6S7UOH<
PO7r\I.Hu&e0d&E<.')fERr/l+*W,)q^D*ai5<uuLX.7g/>$XKrcYp0n+Xl_nU*O(
l[$6Nn+Z_Nq0]s7hs]`XX1nZ8&94a\~>
endstream
endobj
8 0 obj
<</AIS false/BM/Normal/CA 1.0/OP false/OPM 1/SA true/SMask/None/Type/ExtGState/ca 1.0/op false>>
endobj
7 0 obj
<</LastModified(D:20120919101741+02'00')/Private 12 0 R>>
endobj
12 0 obj
<</AIMetaData 13 0 R/AIPDFPrivateData1 14 0 R/AIPDFPrivateData2 15 0 R/AIPDFPrivateData3 16 0 R/AIPDFPrivateData4 17 0 R/ContainerVersion 9/CreatorVersion 15/NumBlock 4/RoundtripVersion 15>>
endobj
13 0 obj
<</Length 943>>stream
%!PS-Adobe-3.0 
%%Creator: Adobe Illustrator(R) 15.0
%%AI8_CreatorVersion: 15.0.0
%%For: (Marc Herbstritt) ()
%%Title: (CC-BY_icon.svg)
%%CreationDate: 19.09.12 10:17
%%Canvassize: 16383
%%BoundingBox: 376 282 465 313
%%HiResBoundingBox: 376.5 282 464.5 313
%%DocumentProcessColors: Cyan Magenta Yellow Black
%AI5_FileFormat 11.0
%AI12_BuildNumber: 399
%AI3_ColorUsage: Color
%AI7_ImageSettings: 0
%%RGBProcessColor: 0 0 0 ([Passermarken])
%AI3_Cropmarks: 376.5 282 464.5 313
%AI3_TemplateBox: 420.5 297.5 420.5 297.5
%AI3_TileBox: 17.5 18 800.5 577
%AI3_DocumentPreview: None
%AI5_ArtSize: 14400 14400
%AI5_RulerUnits: 1
%AI9_ColorModel: 1
%AI5_ArtFlags: 0 0 0 1 0 0 1 0 0
%AI5_TargetResolution: 800
%AI5_NumLayers: 1
%AI9_OpenToView: -461 834 1 1765 1056 26 0 0 113 134 0 0 0 1 1 0 1 1 0 1
%AI5_OpenViewLayers: 7
%%PageOrigin:0 0
%AI7_GridSettings: 72 8 72 8 1 0 0.8 0.8 0.8 0.9 0.9 0.9
%AI9_Flatten: 1
%AI12_CMSettings: 00.MS
%%EndComments

endstream
endobj
14 0 obj
<</Length 10817>>stream
%%BoundingBox: 376 282 465 313
%%HiResBoundingBox: 376.5 282 464.5 313
%AI7_Thumbnail: 128 48 8
%%BeginData: 10682 Hex Bytes
%0000330000660000990000CC0033000033330033660033990033CC0033FF
%0066000066330066660066990066CC0066FF009900009933009966009999
%0099CC0099FF00CC0000CC3300CC6600CC9900CCCC00CCFF00FF3300FF66
%00FF9900FFCC3300003300333300663300993300CC3300FF333300333333
%3333663333993333CC3333FF3366003366333366663366993366CC3366FF
%3399003399333399663399993399CC3399FF33CC0033CC3333CC6633CC99
%33CCCC33CCFF33FF0033FF3333FF6633FF9933FFCC33FFFF660000660033
%6600666600996600CC6600FF6633006633336633666633996633CC6633FF
%6666006666336666666666996666CC6666FF669900669933669966669999
%6699CC6699FF66CC0066CC3366CC6666CC9966CCCC66CCFF66FF0066FF33
%66FF6666FF9966FFCC66FFFF9900009900339900669900999900CC9900FF
%9933009933339933669933999933CC9933FF996600996633996666996699
%9966CC9966FF9999009999339999669999999999CC9999FF99CC0099CC33
%99CC6699CC9999CCCC99CCFF99FF0099FF3399FF6699FF9999FFCC99FFFF
%CC0000CC0033CC0066CC0099CC00CCCC00FFCC3300CC3333CC3366CC3399
%CC33CCCC33FFCC6600CC6633CC6666CC6699CC66CCCC66FFCC9900CC9933
%CC9966CC9999CC99CCCC99FFCCCC00CCCC33CCCC66CCCC99CCCCCCCCCCFF
%CCFF00CCFF33CCFF66CCFF99CCFFCCCCFFFFFF0033FF0066FF0099FF00CC
%FF3300FF3333FF3366FF3399FF33CCFF33FFFF6600FF6633FF6666FF6699
%FF66CCFF66FFFF9900FF9933FF9966FF9999FF99CCFF99FFFFCC00FFCC33
%FFCC66FFCC99FFCCCCFFCCFFFFFF33FFFF66FFFF99FFFFCC110000001100
%000011111111220000002200000022222222440000004400000044444444
%550000005500000055555555770000007700000077777777880000008800
%000088888888AA000000AA000000AAAAAAAABB000000BB000000BBBBBBBB
%DD000000DD000000DDDDDDDDEE000000EE000000EEEEEEEE0000000000FF
%00FF0000FFFFFF0000FF00FFFFFF00FFFFFF
%524C45A8F8F8F827F8F8F827F8F8F827F8F8F827F8F8F827F8F8F827F8F8
%F827F8F8F827F8F8F827F8F8F827F8F8F827F8F8F827F8F8F827F8F8F827
%F8F8F827F8F8F827F8F8F827F8F8F827F8F8F827F8F8F827F8F8F827F8F8
%F827F8F8F827F8F8F827F8F8F827F8F8F827F8F8F827F8F8F827F8F8F827
%F8F8F827F8F8F827F827A8F827587D527D527D527D527D527D527D527D52
%7D527D527D527D527D527D527D527D527D527D527D527D527D527D527D52
%7D527D527D527D527D527D527D527D527D527D527D527D527D527D527D52
%7D527D527D527D527D527D527D527D527D527D527D527D527D527D527D52
%7D527D527D527D527D527D527D527D527D27F8F87DA883A87DA883A87DA8
%83A87DA883A87DA883A87DA883A87DA883A87DA883A87DA883A87DA883A8
%7DA883A87DA883A87DA883A87DA883A87DA883A87DA883A87DA883A87DA8
%83A87DA883A87DFD07A87DA883A87DA883A87DA883A87DA883A87DA883A8
%7DA883A87DA883A87DA883A87DA883A87DA883A8847DF8F87D7D837D837D
%837D837D837D837D837DA87DA87DA87DA87DA87D847D837D837D837D837D
%837D837D837D837D837D837D837D837D837D837D837D837D837D837D837D
%837D837D837D837DA87D837D7D5258527D7DA87D847D837D837D837D837D
%837D837D837D837D837D837D837D837D837D837D837D837D837D837D8452
%F8F87DA87DA87DA87DA87DA87DA87DA8A8A87D7D525227522752527D83A8
%7DA87DA87DA87DA87DA87DA87DA87DA87DA87DA87DA87DA87DA87DA87DA8
%7DA87DA87DA87DA87DA87DA87DA87DA87D7D2727FD05F827277D84A87DA8
%7DA87DA87DA87DA87DA87DA87DA87DA87DA87DA87DA87DA87DA87DA87DA8
%7DA87DA87D7DF8F87D7DA87D837DA87D837DA87DA87D5227FD0AF827527D
%7DA87D837DA87D837DA87D837DA87D837DA87D837DA87D837DA87D837DA8
%7D837DA87D837DA87D837DA87DA85227FD0BF8277DA87DA87D837DA87D83
%7DA87D837DA87D837DA87D837DA87D837DA87D837DA87D837DA87DA858F8
%F87DA87DA87DA87DA87DA87DA85227FD0FF8587DA87DA87DA87DA87DA87D
%A87DA87DA87DA87DA87DA87DA87DA87DA87DA87DA87DA87DA87DA87DA87D
%A852FD04F8527DA8A8A87D52F8F8F8277DA87DA87DA87DA87DA87DA87DA8
%7DA87DA87DA87DA87DA87DA87DA87DA87DA87DA87DA8837DF8F87D7D837D
%837D837D837D8327FD06F82727522727FD07F8277DA87D837D837D837D83
%7D837D837D837D837D837D837D837D837D837D837D837D837D837D837DA8
%27F8F8F852FD08FFA827F8F8F852A87D837D837D837D837D837D837D837D
%837D837D837D837D837D837D837D837D837DA858F8277DA87DA87DA87DA8
%83A827FD04F8277DA8FD06FFA87D27FD04F8277DA87DA87DA87DA87DA87D
%A87DA87DA87DA87DA87DA87DA87DA87DA87DA87DA87DA87DA87DA852F8F8
%27A8FD04FF7D27A8FD04FF7DF8F8277DA87DA87DA87DA87DA87DA87DA87D
%A87DA87DA87DA87DA87DA87DA87DA87DA87DA8837DF8F87D7D837DA87D83
%7DA827FD04F87DFD0CFF7D27F8F8F8277DA87DA87D837DA87D837DA87D83
%7DA87D837DA87D837DA87D837DA87D837DA87D837DA87DF8F8F8A8FD04FF
%7DF8F8F8FD05FF7DF8F8277DA87D837DA87D837DA87D837DA87D837DA87D
%837DA87D837DA87D837DA87D837DA87DF8F87DA87DA87DA87DA827F8F8F8
%27FD0FFFA852F8F8F8277DA87DA87DA87DA87DA87DA87DA87DA87DA87DA8
%7DA87DA87DA87DA87DA87DA87DA88352F8F87DFD05FF7DF8F8F8A8FD05FF
%52F8F85883A87DA87DA87DA87DA87DA87DA87DA87DA87DA87DA87DA87DA8
%7DA87DA87DA87D7DF8F87D7D837D837DA827F8F8F827FD12FF52F8F8F852
%7D837D837D837D837D837D837D837D837D837D837D837D837D837D837D83
%7D837D7DF8F827FD07FF27F852FD07FFF8F8F8837D837D837D837D837D83
%7D837D837D837D837D837D837D837D837D837D837DA852F8F87DA87DA87D
%A87DF8F8F827FD14FF52F8F8F87D83A87DA87DA87DA87DA87DA87DA87DA8
%7DA87DA87DA87DA87DA87DA87DA87DA852F8F8FD07FF7D7D52A87DFD06FF
%7DF8F87DA87DA87DA87DA87DA87DA87DA87DA87DA87DA87DA87DA87DA87D
%A87DA87DA87D7DF8F87D7DA87D837D27F8F8F8A8FD14FFA8F8F8F805A87D
%A87D837DA87D837DA87D837DA87D837DA87D837DA87D837DA87D837DA87D
%27F827FD06FFFD06F852FD05FFA8F8F8527DA87D837DA87D837DA87D837D
%A87D837DA87D837DA87D837DA87D837DA87DA858F8F87DA87DA8837DF8F8
%F87DFD16FF7DF8F8F852A87DA87DA87DA87DA87DA87DA87DA87DA87DA87D
%A87DA87DA87DA87DA87DA8F8F852FD06FFFD06F852FD06FF27F827A87DA8
%7DA87DA87DA87DA87DA87DA87DA87DA87DA87DA87DA87DA87DA87DA8837D
%F8F87D7D837DA827F8F827FD18FF27F8F8277D837D837D837D837D837D83
%7D837D837D837D837D837D837D837D837D837DF8F87DFD06FFFD06F827FD
%06FF52F8277D837D837D837D837D837D837D837D837D837D837D837D837D
%837D837D837DA858F8277DA87DA87D27F8F87DFD05FFA87D527DA8FD05FF
%7D7D527DA8FD04FF7DF8F8F8837DA87DA87DA87DA87DA87DA87DA87DA87D
%A87DA87DA87DA87DA87DA87D7DF8F87DFD06FF27FD05F852FD06FF52F827
%A87DA87DA87DA87DA87DA87DA87DA87DA87DA87DA87DA87DA87DA87DA87D
%A8837DF8F87D7D837D7DF8F8F8FD05FF52FD05F827FFFFA8FD06F87DFFFF
%FFA8F8F8F852A87DA87D837DA87D837DA87D837DA87D837DA87D837DA87D
%837DA87DA858F8F8A8FD06FFFD06F827FD06FF52F8277D837DA87D837DA8
%7D837DA87D837DA87D837DA87D837DA87D837DA87D837DA87DF8F87DA87D
%A852F8F827FD04FF52F8F8F82727F8F852FFF8F8F82727F8F8F8A8FFFFFF
%27F8F852A8A87DA87DA87DA87DA87DA87DA87DA87DA87DA87DA87DA87DA8
%7DA87D83F8F87DFD06FF27FD05F852FD06FF27F827A87DA87DA87DA87DA8
%7DA87DA87DA87DA87DA87DA87DA87DA87DA87DA87DA87D7DF8F87D7D847D
%27F8F852FFFFFFA8F8F8F87DFFA827F8A852F8F827A8FF52F827A8FFFFFF
%52F8F827A87D837D837D837D837D837D837D837D837D837D837D837D837D
%837DA87D27F852FD07FF52F8F8F87DFD06FFA827F8527D837D837D837D83
%7D837D837D837D837D837D837D837D837D837D837D837DA852F8F87DA87D
%A827F8F87DFFFFFF7DF8F827FFFFFFA8FFFF52F8F87DFFFFFFA8FD05FF7D
%F8F85283A87DA87DA87DA87DA87DA87DA87DA87DA87DA87DA87DA87DA87D
%A87DA827F827FD07FF52F8F8F87DFD06FFA8F8F852A87DA87DA87DA87DA8
%7DA87DA87DA87DA87DA87DA87DA87DA87DA87DA87DA87D7DF8F87D7DA87D
%27F8F87DFFFFFF52F8F852FD06FFF8F8F8A8FD09FF7DF8F827A87D837DA8
%7D837DA87D837DA87D837DA87D837DA87D837DA87D837DA87D58F8F87DFD
%06FF52F8F8F87DFD06FF52F8F87D7DA87D837DA87D837DA87D837DA87D83
%7DA87D837DA87D837DA87D837DA87DA858F8F87DA87DA827F8F87DFFFFFF
%7DF8F852FD06FF27F8F8A8FD09FF7DF8F8277DA87DA87DA87DA87DA87DA8
%7DA87DA87DA87DA87DA87DA87DA87DA87DA87D27F827FD06FF52F8F8F87D
%FD05FFA8F8F85284A87DA87DA87DA87DA87DA87DA87DA87DA87DA87DA87D
%A87DA87DA87DA87DA8837DF8F87D7D837D27F8F852FFFFFF52F8F827FFFF
%FFA87DFF27F8F87DFFFFFF7DA8FD04FF7DF8F827A87D837D837D837D837D
%837D837D837D837D837D837D837D837D837D837DA852F8F852FD05FF52F8
%F8F87DFD04FFA827F8F858A87D837D837D837D837D837D837D837D837D83
%7D837D837D837D837D837D837DA858F8277DA87DA827F8F852FD04FFF8F8
%F87DFFA8F8F87D7DF8F8F8A8FF7DF8277DFFFFFF52F8F85283A87DA87DA8
%7DA87DA87DA87DA87DA87DA87DA87DA87DA87DA87DA87DA87DA827F8F852
%FD04FF52F8F8F87DFD04FF52F8F852A87DA87DA87DA87DA87DA87DA87DA8
%7DA87DA87DA87DA87DA87DA87DA87DA87DA8837DF8F87D7D837D52F8F827
%FD04FF52F8F8F827F8F8F87DFF27FD07F8A8FFFFFF27F8F852A87DA87D83
%7DA87D837DA87D837DA87D837DA87D837DA87D837DA87D837DA87D7DF8F8
%F852A8FFFFFFA8A8A8FFFFFFA827F8F827A87DA87D837DA87D837DA87D83
%7DA87D837DA87D837DA87D837DA87D837DA87D837DA87DF8F87DA87DA852
%F8F8F8A8FD04FF7DFD05F87DFFFFA827FD05F8A8FD04FFF8F8F87D83A87D
%A87DA87DA87DA87DA87DA87DA87DA87DA87DA87DA87DA87DA87DA87DA883
%83F8F8F82752FD06FFA852F8F8F827A883A87DA87DA87DA87DA87DA87DA8
%7DA87DA87DA87DA87DA87DA87DA87DA87DA87DA87D7DF8F87D7D837D7DF8
%F8F87DFD05FFA87D7D7DFFFFFFA8FFFFA8527D7DFD05FF52F8F8F87DA87D
%837D837D837D837D837D837D837D837D837D837D837D837D837D837D837D
%837D7D27FD04F82727522727FD04F827A87D837D837D837D837D837D837D
%837D837D837D837D837D837D837D837D837D837D837DA852F8F87DA87DA8
%8352F8F8F8FD18FF27F8F827A87DA87DA87DA87DA87DA87DA87DA87DA87D
%A87DA87DA87DA87DA87DA87DA87DA87DA87DA85227FD09F8527DA87DA87D
%A87DA87DA87DA87DA87DA87DA87DA87DA87DA87DA87DA87DA87DA87DA87D
%A87DA87D7DF8F87D7DA87DA852F8F8F852FD16FF7DF8F8F87D7DA87D837D
%A87D837DA87D837DA87D837DA87D837DA87D837DA87D837DA87D837DA87D
%837DA87D7D2727F827F827527D7DA87D837DA87D837DA87D837DA87D837D
%A87D837DA87D837DA87D837DA87D837DA87D837DA87DA858F8F87DA87DA8
%7DA827F8F8F87DFD15FFF8F8F82783A87DA87DA87DA87DA87DA87DA87DA8
%7DA87DA87DA87DA87DA87DA87DA87DA87DA87DA87DA87DA883A87DA87DA8
%7DA883A87DA87DA87DA87DA87DA87DA87DA87DA87DA87DA87DA87DA87DA8
%7DA87DA87DA87DA87DA87DA8837DF8F87D7DA87DA87D7DFD04F8A8FD13FF
%FD04F852A87DA87DA87DA87DA87DA87DA87DA87DA87DA87DA87DA87DA87D
%A87DA87DA87DA87DA87DA87DA87DA87DA87DA87DA87DA87DA87DA87DA87D
%A87DA87DA87DA87DA87DA87DA87DA87DA87DA87DA87DA87DA87DA87DA87D
%A87DA87DF82758837D837DA8837DF8F8F827A8FD11FF27F8F8F852A883A8
%7D837D7D7D837D7D7D837D7D7D837D7D7D837D7D7D837D7D7D837D7D7D83
%7D7D7D837D7D7D837D7D7D837D7D7D837D7D7D837D7D7D837D7D7D837D7D
%7D837D7D7D837D7D7D837D7D7D837D7D7D837D7D7D837D7D7D837D7DFD06
%F8277D847D52F8F8F8277DFD0EFFA8FD04F827A87DA827F8F827F8F8F827
%F8F8F827F8F8F827F8F8F827F8F8F827F8F8F827F8F8F827F8F8F827F8F8
%F827F8F8F827F8F8F827F8F8F827F8F8F827F8F8F827F8F8F827F8F8F827
%F8F8F827F8F8F827F8F8F827F8F8F827F8F8F827FD08F87DA8A87D27FD04
%F852FD0CFF7DFD04F827A883A852FD61F87D7D837D2DFD05F8527DFD05FF
%A8A85227FD04F827837DA87DFD62F827A87DA88452FD07F82727522727FD
%06F852A87DA87D27FD26F82752527D52F8277D27F8F8275227FD2FF82783
%7DA8837D27FD0EF82752A87DA87D27FD27F87DFD04FF7D27FFFFF8F8A8FF
%FD31F827A883A883A85252FD09F827277D83A87DA87D27FD28F87DFFF8F8
%A8FFF852FF5252FF52FD33F87D7DA87DA87D7D525227522752527D7DA87D
%A87DA85227FD29F87DFF5252FF7DF8F8A8FFFFA8FD35F8527DA87DA883A8
%83A8A8A883A884A87DA8A8A85227FD2AF87DFFA8FFFFA8F8F827FFFF52FD
%36F827527D7DA87D837DA87D837DA87DA87D52FD2DF87DFFF8F852FF52F8
%F8A8FFFD3AF852527D7DA87DA87D837D7D2727FD2EF87DFF27277DFF27F8
%F8FFA8FD3DF8FD0527FD33F87DFD04FF7DF8F8F8A8FFFD75F82752275227
%FD04F82727FDAAF827F8F8F827F8F8F827F8F8F827F8F8F827F8F8F827F8
%F8F827F8F8F827F8F8F827F8F8F827F8F8F827F8F8F827F8F8F827F8F8F8
%27F8F8F827F8F8F827F8F8F827F8F8F827F8F8F827F8F8F827F8F8F827F8
%F8F827F8F8F827F8F8F827F8F8F827F8F8F827F8F8F827F8F8F827F8F8F8
%27F8F8F827F8F8F827F8F8F827F8F8F8FD7FA8FF
%%EndData

endstream
endobj
15 0 obj
<</Filter[/FlateDecode]/Length 12902>>stream
H‰ÜWýrÚ:ßà´Óé™mcÀ†þ¤IٛÒ4½Ý#lº'G–IÈóì›ì‹í'lƒá#½mÃݦ!XçûœŸÎ9~û÷nÿ¸é‹!9¶%"{û¶-	VB69EÆ¢PI}"ï!«Z(S³ãÆ"C*xÐñTKç/°ôÐG"‡ M•:Bù# ]SÅPÛíã֗õ/"³ñQj`V½Pª¬2²J
ËÑdÌg8é£&Öl׆³–ˆ¸Où¸%Èvj¨ì–Q¥VE¶¥Éi"«<…jÂU)¤|'‹¦"«®	ö`B†
ԞcŽ.ð(}!Œ‰{ÔbØ»ËAøÕÁ)e"b…,KÇÝìXåA+¢Ì¿Œ¦C9°ëu}lŒÊO!èµú»>v)œô‰RàԹ띵²nÀ¡ùÉíBð¬É;¿%j¥ôI¸!2ÍsM¦ƒ"šø+å'æª;ð™ùžpB@†ËÒdËEnIsT'¦/ÓDf"Ü7Ð¥à$ÎESª~\™J¥TŠ?cJ/bD~âT–>ªÇɸ>aɑ'?eØäÀüXËϘáË1QPNÁ"eÐæ¦ ÙçxNäÒÀU@øµ¸1>Wjrí
(³@†UªLj±~ËFR›Öò3V­i5©~Ã."ìJÒ1åÄ;gp&©¿,£SFnüa(¸™ßzú{
A+Exâ9À§}'C©pÑ‹¸ßSùPcž€i€㘶øn( ±÷æyEêJʵÎÜ¥¡¸ƒ.‹€t&EtøHäòñU¿–Ø6t5üƒxúÂ^boòH¨7á"ÃcBïGT'¦ÁÑVm›$(&'°yLÿî–>!#¸[Kñøôã¿Ë¶ÃáÇ¿G!VSáG¨øŒ0"¹>cì6Ðe˜c‰Ìyª?«u¸"ß):CSÌLÎé1dsý€˜ÒhDËS[Û2¤=a5¾D¸.t7ù˜éºE|¼–+D̾[wßÓø"¨%£p'®…`ý€<RÌÊCÂVL$bFJ¡®àW<NÛº¹˜vD>k
ºÔAZîÍVZ0þ"6ژ1:–8˜Pï93¿%ô%ÏZ‹å_'ºùt(
§K°eNºX*ê1ҟC¦Û´é¼Œ(÷À¦9.Ôiÿtç"¨GMššQ­&§F ¿Ð[@3϶ëããí}¼SôìUsFÂ\ñ7.î¹y@\þk_A;ÄÒÿv"Š—xJл\±Oa )O	]å`gƒ6̪Í_âŸ[=¨[åŠs³à¸N­\…/5«îڎlN¥æ$õ¶™KG9<Ìáá_ðå8º‡9Œ.Ð×o%äÃñm/gôû¹¢é®è}aÀ_'$fåÎTu¡[ÃÕËi«Ýáþî®îXf¸}Ì­í^]/×m-üHͽ¤Vç4TO
´§áøTX¥˜#Y«ù[rŠV7(OœM÷=XÈqîí ˜>nôõô"†åÜ<תU»ŠŠ04û:'»3òô¶‰"Ä?'äíÅù%lF,ÿÆO´Fûð¢ëGþaÊ80븍垧Ï0‹†zb>KVó ¡›RâØקL‰Â>"ÀžêÁùŸôÃú>?¤?jôNN_Û
Ïk|òîµÝð½Æȼ\½¶#oyØ
Î<Õ¯rEx•ý'0l÷9㓽¯Oï—<Þ¦­Ôûè»gîa†öI‡'"aÌú>ùüQšÖ
{þ«Ëµw@ë×MÂûd$½½ÎO"
ÅbIVr\ô=ø?¥Ú/ˆ‡2ÖÑ0Ø»üå_[þ•˜ßýP¸¬gE´÷õÍtҒP~lÆ^xÁfXR<"ݍ¨ðÏËïì†'^݇_™…ŸVÔ¼ ÀB®w¬_\Øï¼ÙZf·›ùðpàÁ®˜¾ßÀüŠW:‰a½†Ð˜íà0<Ôàt?³¿3áÝé…~Wž¸àäðR"zÿl"…kxiØېrèÖáŗâg¢à½à/˞Iz{8ºµ	2êý_Œ?Hßì£-qÿ czêò"Ðñd÷òcƒ='ÙÁ =õ{½÷ÔW"¹î"¸½Ï|g,e·|`Á̟ÝFv£Ì©ªÊÃs¡…'UðœŒÔ•¤cÊwFק%ÄáDµÀV˜Cñ¹ú9¢zýüÄ©';ò4%
ûð†Uvj•íB¯˜2êÿè|m·÷Æ^4%<™	y«Z(J(Ý5;§c'	Û
'!(j,Puën:l»@Ÿ'3Iý¾'­e&ke«²…óL'4"j)íf«Œ§Ly`ª¤YÚPNgƒZÃÝKwüÒ®^ĈŒïs‡ûäá"ÊP½L¤O<Á3N½jA;vmkѕ»'r¥×–gï2ÌI›0öáA-
áZu£¥R±^ ¥eú"a|¢Æ©¿H͵2:6%aÁ~CC:¤JÒWX'íR¦&›Åv–s	¨JÕu6Ê°fån""#›ù-¬=½<eywàt4
‰Úi3M²ˆ®U«ö–"ïÄ346•ŽOkWÍûfI>Ç2‹!³Vn0§áºD,å
N]/zæb¦7;–…º'"Dκ&
}ð©Â1&žÆhxÓ"àµ6
Ð9æã	êŠ 
å5Ûµ2©@óûôñ™Wª•n™ÿPoBøˆý÷?ðYë"âreñ²-;"­a×¢÷†8s"¤Ú'¡Z	tk\, {–ÉKPÔì­¤³6¥
,ý2ÂSK?Ó,žÐ0`x~å]Ú*Ž)¹S[-x¦Å­ŒÔŒIâSm)'¦$¸i
ŸŒ"¥'þ§SU0ß²¦s6Ђ-ñpû%'qÝ­|Ÿ—[Þ¶¶²~̼ñè›UÝÔÒ5ÛîY¡¹–-h[·2¬™"Å}	c‰DAzČÈüWáwŒÝBS¬$ÛÜÇn(¹‡<æÞ¢nëP§Ø#M>f;™MØ+ÜåÍÝôQðl•ìÌzH.o±µÑÍ×Ñb©)%A¥ç¡¢ó'A_iC¥D¤å)hUÛkê1 OLF$c¨L¸Áf§Žpr™€›		ýz¼DÌNÞáˆÕr¥ìnf-ƒþžœvò.°6²=š®$æa€acõæ`Žú(\5"û:
pÉé4bÝ)>ÑLW'
"…z8T°dQ"'EK«úD悄"ÿ'^­[mãZø	úʙé) 	¹@(…NB¸dZ(%Y´e˜¡¾(‰&Žå%ÉPxžóýuþõÅΖ_âزéü`­`}[Ú÷ýí‰úҘ
Y2"€²–c׆҂g.µf5`$
'ÔÚçDè­u}˜2ß¹ïNþ\2Yï$J056Š[|zŽ…ÄB°ˆÀnÛ#ՔچCx*£¹GE
57øbn4wBoz†o,ÝØ$häÙ՘f֌Νd»ž˜ùI4S—nÝCC·.m·Î皝V³<SïJSõ:Új‡)©'Ç2‡ï±b†YÌ)¿Gª§—(bgg·<USâY/>kÀÄöÿ³%#¾gyËؗ'e6¶WÕ.¨X:"Ú÷±u"YŠí¸€.É7ì€.cP%•é+£Ô5¼Œ¢ZÕamµjk­Œ˜¾À¼ö75«a+"Ž7IuÊ4T~ÃqB^ ây¶'†œx½žsô	gewKƒŠÂ±ôÓkÇgÄ3!ȳDoPl"F¿SsàŽ)'Þ-åè,}¬y5dNTLuú$Öüq¶<R@PG)¹vDÁ%6:ùpzÕmî¡ÛµÁðÚnì´v·¯õzëv]Ÿêi:&Ž&ö€™ƒ¸.Ž?¼jùÊn½Læ)¼áº4Nõ ³¬€ÂöÊy~ä ïZì0í獹ä-ß¼ª»²³¤Ô³ý/ºÁ¢ùÑ€$oùo2ŸUÁNlÓñ¸ês-¦'ÿÕÔ«¼"ºP;"uZýÈÉlç ©-s–f=ÉÒÈÝv6pi¬f¦$>eôd— mièԀ†'õ÷9ےOBß	êjü«0sÙx'éeá\<1â-6dÙ³æ(MÓÉ¿dìŠ*÷M®1LBlÇccí†YYÀâ^²"én™¾sƒÍ¸L_SòÒp/i%Ђz¥±¬˜'rÀQÑ%µ.Oh]i]»¤uv§P+i0]rKœ\¡9BŸ–*':ùYô2KX¢icLµÑÎ5ØÆcIÔˆ-¦z†`17¼t·)Wê
D"ƒ²ŒD0ãášk&…˜¥á•z‹ÙU
Ù1¼ê}IœÆ[&`#	yk&5·,W׌çX‰ý)[+nu/ÄM‹ld"b?fqOÖÀ'r¢Oz‰'üó¦"=…«lŽ2l¿ Š,‡©)

,՚é±áìö¨Ð"±DÆÍ·Än ç:1ÇçAQ•€&˜f¿p&õ][cŠژ"‰[äIÏcUèZ.×%'M¡_%('="ƒMqAO.‹ûÕZßg֍&&fq	Ä´ ÍÀ%q":õlB 2‡ž¼4—Ú»»zpb*mwôÐh$ãyÔi5ò Ißµ÷²›þ²ó2i0@À‹†ïè& €ž±¶pá,àžgç?-a‹§#\‰›+ËӉZFH–f±L'B>܁†ÂpmƒÙ‹[²Ô.¢‡öÑZw°½.卨'QŸXbY•áõé	0Ã÷ÔJTkêpM›V|<"Óqô莨G©£Ž>'ºNôq‹É÷ÒHPÄÙÜÒû*:éú'¾G®Ê\NÆË´P9V©ÏMl_<òqB¨?ê¯lʅǗCôøê2  Hš€®R$%ôX$ò!!çn¯^{Ê[Nuí9æӕk£M+'	Ô¯]CÄ)C½äÆù%VÂ'z)•S^]ÁÕrÉó`G0CÑ—ƒ¿šP'‡‰zNp/.òÇÎm£Ùà¾;'Y¦ktË	ÄW`šè%Ð<,ÐÅJm¶ºƒ.ÇEAJ"¥½"ô<§+''>ÔÖº|	'ëq…ú§W—èý>¸‡\Š"Nƒˆ‹äš+©UFYwmjby
÷Œ/\bÆ=ٌîñ)#öÝpJÎHHkšq¹:áIz*34îñ94C†ClM
paxM¶/1Ø#zjT\a‹2ہ_zØõÅf%tVãÌêÐ2{/û'w9}úàrCåq5c&"Qng÷xà8¾ÚÐ(;¶‰l¥G†g˜@áÁÙqýñ=ŒªÆ†ðE á<t¡Eu4Žrƒ.''2k$çȉd®	Y2¯­E^³d^'ŠuY~oQ§ªɓT¹8õtCzçˆ:")".sî':$ÜxÖþè\æ
2ü1z•ˆÓV8_ý	ssÄ!âz
0å
ƒ";Á.21™£¡‡‰5…Q…à¬MÞׇÙFáp:mõé̟Cª¢kÌ°kÃC¸à'¯ÞDp¢àîýø/¸CVkây¢¾Éççè½ñAò0c>G ýTE½*¸}EÑAkƒæ4ÿñݚÊêùZM~üjq'C-A!þô€­™ªø®‰g†+[Õ"U!ç-F<ý†Êî'Ü<ƒa7Š^¹Çdû=^"eo¡ ´jϐ9¶Z3$AÆ$Ít•ßµ5
'ۊK
M™0•ì[÷ÁÌ1"3G—é—L­qׂ"H¥ºN.Lébdà8W,^"n]ª©ŸrnñӐ3Ð9Uù'ŸË‰'"ñ<¬7«©€@>ƒÖù,b&û,£WÜ·P°®Ë¨€†Kv{%}P<|"
¥…¶"k©Õsp訝ì>¼¸u<–j0:‡ñü@ÙlDc¢Ÿ/¦® :µ¸Ý¬ì­ï£ÍõyŠ÷¨ˆ¶KãGŒÌÏ
6ã?óH¬\±!Wd2eZ‹Ú¥J‰Õ«Úhëø"ãGžgIYíŒ	ôŸ1-FB[N¸U‡T¼g"
´ÑÞ)ài#¨«!y
몭»|™×•äµæôÞe¥CœÌ¹¦¶ÜÏ©K­)¸ç+×Ò&oˆesLמ_Æ0ðw&×Õ>˜Kk[´Ð ¿Ø*å¢LÑ"2Ÿúè@Å¥ÑÈÐéòl¯æ=ªÌJ…ØL[ÓOÆRz#S'L[©/@%¼\ZvTç6¯	~xÖ(MЁrœôÀÕÖõ˜(Áì#˜Ô?·u‰"‰äÑԟ›®AœE÷ÚGkp£h
ÏVÖÚý/A»c׆!­V`݆ü¸½}×fëŽ`ÿ
Ï^¨ç"_ÐkT돃N»¥Oå­‡í¯»o¯ÍZ½¶q¾¹ñv*šòW£õæãëftð1ú¥ö›oG¢×ïÎÎ~¹:0úãú—Ãè´±qpµ3­¬7Ï*[µWW/^V6go*ë7{•Í)£¯ãjeÃ=¬lžîW¶êçzíà˚z¾]9ZÿØâ
~Êõg­·¾6{fgçfg~ófëë	ÝýÔ¬Ûñiýì½xÉØáÙÝô.~ÿíÝ?윽ùT=¡7­ëcv{Sïߜ|t¬íÿtwÝÅ+Í_Ÿgx,0Ž±Veóú¯Ae«³Õ©lXÕ¡´ª#¿W6ïìveÌœÊºèiÚzÒ´Öæ•üÕEn»ÊŒÃ½³_ÿŽ
zñR™Ä+¾ê7^þ«ŸUk¼sÚxûËÙ_ðï©S·ÿý¥šñž3¶Ï¯Ù­ÓyW¯µ†Sc?äËÏÍßþÏzy.¦Êƒø
¼´¸G@´n<ZÜZmÕ:ªV«=­îûÿB@ ˜ ž¯rF$Ï»GË톔¹"C–¸×ý¶å½Ù`¸;ø2EÆ©;A…ÕÃã
:ގ&ï&èQ—X1ýÙx׀GM´äøš…dhŠîÝ~Rˆº¶Ò®L"?¬ ¾ä«¢@£GwЈ˜ 2a…þrÑ{"Ô^XÆn~ÂÉ&	

o¯%*ÔÉ}	e%AW¡?Åâ¶OÖ´°éðùöLö©°:ñ©ë;¡B›.'"ŠêÕð¶zGP'3	÷êp;ºë6e¨ç4""'°vdèºT±±&¬6@ÒAƒ¾nÇ1®G†6$¯c=Ôu¨Õ±;Ç:W AK"ÿÃ
ÈPÁÓ÷%¿:
"Ô^˜Fl¬	kôjµ•£@£6‹ˆh
«v[‡B]ØâMÚY[¼wˆÐb+Ö¥jê0AÕ§ÒógK»ÇÆî\YÿNÆzOt-M¾™z»6CkåÆH…ön"¦·'`p CaŒuä@í»uK†–í‡X­ÿ#Bï¿%*ÔÆVƒ›µŸ¬«0ôÇÚæ@†VÃãZ¡ 2Dh»üQÖ¡Ð/8ö±m¿Ð w Æq2´p´ço'…¦;N墨v݋ɚ­ƒ§€˜£@%ßS6¶Í#¨5ë:ð·ÇTèÒÞ®å(Ðç(M_|$(Œ1{£óñ™`~¢Çãބ
]-D÷_´^¤Ú'Ê1fÎÕgïí[et»m*tö˜'Æ÷Ja:µï‹:Tž.RLb{灌õŸ@ïÓîÍXêe!4½5wšÄªïW¡Ÿq¯	ʾ
íojcù\Ÿ+ãâHaQ†NKa#pì4ù½Ù¼'´*PÑ-ùu(¬É¡]äÝ5÷©U)|"ÈWñR¸ð¥c¡
B£¬=Ý/• ´Â˜ Ÿ»GPÙ/‰VФër•–>¨Ø©ÕðVm¼|_¡öJ/ͼñ–ß3|âgfºÕ:2p2áù÷šüµàI"‰,h·[õÊ-š.¤Ô½¤ÜŸ´åAÔ²aݞøj¢@»ýjójÝÚXÂ}ԙ§ík	Ü¿–h·ð˜ÿܛnõfè]CùzílÝM»€³	'oS€ùr`nÕûÓJUÝ"VnñD"o+ û7 Ònkàé&þçh±ÓûxŠJyÚ×M0p܎h·K0ê
¼¦[ÝbÏ·`´|óS¾~Žƒq'¦ÝfÁ$:‰Sn'[¨KÐ[Pî§n.þÂ×)·3—sŽ´ÛG®Ú²W¨{]qOþƒòõÜÃõ—U'ù62þi'SûÍbü®É¸<4S¹á&ã.a9½ûÃKٌrk®|üþ‹I	•%ùVð<Ã
"âÿ¶h÷#_*ùý`¸Í¼êÆ+Zfힷ}¹Õ®¡T¯LzÍV3éy'S«¥i9CUp»96Ú»ò…¶xÛGËåÝ@JáÿB>|Íçs¡ª~ö¸V?{a¿diÂ
Ï@v"]h¯|+ëNgý5Ôëf¨ûqÁ²w@ë,®o)mgu">Ò3Ì@»—D+Ö[;ïJ7Çe美õ}{"FÞ½lŠY'¡B¿G‡Úó	
»˜†…v®EÂÁøþ£>¥A_, Å@ëûs§Ó¡C·»"o§AÃ4VzïµäZüÂÌkw¡Â㍍ձÛäBQ´Q p›"›Ã3*ô‡hK2b1óT(Ú¨Pys˜ëP¨†]С±F«G‡ÊóÕ¼6VžH&4]['^u$ü*ýMó"õïä
£þ2yыÂsí²ßyšÊïäjfþZTû†?IÝÂáÌ]üýӇšÿ"âr´¬žñYÎßáüÚ1Tý¢ÎÐÞ²Y×Æ|zñýÈO<h2´à²ç\ÉâɳücÖX˜d|%²èÝù"ïb*à^"çNÞèGG^ED/fâÅNþÓɪǴw§ùò+-=qᏇwœ4Úe¿h
DÎH¬zøë+Å:ÊÌ,Ǻ0ó˜vυÞw,ŒdøI"­…Ò~BÉ/ù•Cµ'÷£¾åÒ·WÅ臌ŽU¿¦ËEѯÉèú¡^y¢¡v<W 'ÿàŒ]?ç¿ÉAޒTᕍ¨¥J†•æäõŸ=j˜ô]i,z0$ý¦§`Vžwr°ûkëÈÒãJ‰dzd7ÎÞ¿ÀòÖv—û>´ü¹0½8s'€dwÕ/獅—žàê¤ôôýk iŸ·±×xC'Õ(žÐDÆJÇ‰¢'–•}ÿž**¬íèPmWdœDÛIÏ]SV79+•Å‡ šÈUk¨fcMÊaªÖª)Ç¢tf֞ԚlãbóÛÆÒڑ®•Sъìc	,vŸOÖ
وÞ2Åêšarœ«NÓ¬nŒ1註ÐofBïÒP—žRcG‹de¿!>6ÛQ£>eèÈxÞq듼›ñ›t&e6óCy`·ÿŒ—-|99¸à¬W÷k5ÉM	‹irU¤.¬Ét‡Ê‡*¼°"ÇÔ¯ØSþœ‰"6ƒd>ªdà-R"¼o'¦0Ý»ŠÅp—›—|ƶÖ=κô»Ôª·£5&â̈OŒºw‹¦ªŠ²oLûw^ä¦7®Òӓ>]ç'ÌXq朱Ò3·µH°ŽÉBñ¹A¼BJ›æh#.'âWêλ y@{~ÞXŽ33¿ÑƒgFº+ü'×±é¤ó;ÅrÑ%=…ürõcxC9/—¡Zž<öæÚô~Íbgæºk"|K¸¿f1SE»Öb'ÿÁh™}fcZ\ù\oL-BæéXŸ•j‰Kû·"7z«–Ü K°%"K–uÌ8`g¨Ð§ý—²²äÝRõܸu‡òP<ù·dcÃ7ÉjíYçüÚg;oIð'%M™)èºPËÂnš·]Û%¢œ«gÓ…ÿß6¡¦=Äƞ
¹Eí3;‹nGÚga¶%AñÔR¿	 ¡2ñÒÍò(ϲ«ÀTºÐt¹(3Ìh÷Ã\S>h	²,›Æ|ã;+&ÒÞqi€«Áªü;Uþeùò`­ßÞç"éu¹Úèç&sÌ
+­òãQ+ºïöœ7·,ü'~»w^Ÿ-Ï&$ã½fÑ™âó†6ö:cY¦8ÉXè˜/c]™â˜±ðª]Kñï
žâ"%Môn'7Â7	»¡Â:†í¹z´9åãb»ïŠÅž‡-Èv¨#S&x'«:±ØмÅ:¬MîÈ	K¥R-,vÛuªj¶£©‹ŠÜÄ&¾‰oÀ%Z-šA'i>Pr¿)ÝÕÿVÈÜSµ$Ô&X¥ìyœ¨ìQÜT9à§f1öÙ0'c(Sû¾H(²mf»K"Y/>ú(-&š{Ó(;,c2>Ôåü0}êƒu¥ÏØN«0xP‰Žµó$LkƒUÔÕ^iŠ‰k'áuoƒÿ–/b'íù?qŽ"y]5·?²V–qžh1xß3(¤ér‰B¬ðÀcՓ~÷šÅÔèd'÷©­Ž2ËÊÖÁݙ>$SŽÓì¬WéZ"I|'~î«9<F<˜áTGĕYVFAŽ÷ߪîê®þ°~,™•™'ɐºˆˆÀ·üt^UßE?äoÆX‡|òöÓûPk{MÄU­õa†Â6ŒDïøjg'ýÞër¾ÀÒx°ÀÄäSÚɐ4Æ>bew-¥Pˆ(p➲ÁºOá$ò*ÌÃ셓TÈFSP>,µ‡ˆÚ³]o,¶}RöÏšÝ˜3ÚD²'˦îÐ0J'ÐÝ0Œº»v–˜Wm´TÑýµÅ¥|gÓJ}Á
¨h£Óå8Fm4ð]^ÁÆ´ÔIô»{o4Ø`+=9xÑFPŒûB­!•Ö›{Úhl§"™¬f¹½¹ºv?÷!Ž®6cR•"FÑBGe}ȳ!™Sžá·Xz:O\ÚSä\¥sȆ%Hc'ů£h×\6Ó®GÑBØYgSÞ<qÊÐÃïTíÍÊÓ¬ÊÖð¿n–{:³~Ï]²¶Vz^³˜|Éjªk€õƎkÆá~m°Èz¦wƒBuÍIX¼a¤8\kÏE!µÒÁñrÎñ³#×Ø]¹+¹Ê³\K®1ŒãÓpÛß³´VÌQñ¿– Õpìo(Ü4±š_ÿñþþ鋫…ŽWVC&ô÷,-$ö	¶£¿Ç{jø¡bcó *pöW bGŹɳÉpQëSÄ1¸j(ÖBƆ1üIïj(ÐÂ|T‡Ý§Ô0õxE@5d½$2\›¯r¸sú{f²î¦Óÿòºù![Bù(ÿ5K©1I¼çÐh¹£Óu¼%	æ™ÝܼLnc÷Lîž@ÅNĝÔÄ!Ù˞ŠË´ ¸_ßôò¼-OL"RJØD˜Q¶fBl5©#-[ì'",ïžW*w¥D˜àë"Yº»7ô®¡›`ÿ%ï/ö§>¥RrÈe{KkXJ)Ém´Vó…ÙsWJú'-OøÀZ'L2Äh'U&¦8ð‡½XŒ'A/k­U0Ù_WðÄy¤&'Ï7)"¥'®…¢É…úBkÓü•IWGÌqF=MJËåÕÝ´ö·7•o›Jõ,øý¹Ú¹jU¾§× ÈÕNátPþUtÊ¿*)ðm¦Z*¦þ)•Šéz€=,ØKè/™2¢áU ¿»ýH¥Wß®ÝÅß¡›Hºùí3YyÙß,—¾a*×øsáT9ßW©¿²úvŸoáã5ZúÁi%—í"iâüŸ»&6/xÐãi<tá›ÃÍO"EA}~Põ-Í
š©vŠ÷TP³/fؓ@èî¿æ˜ôE´–<¾…Ã7èr•O¬,oygéYà£þ´qn­ýŃ^ø£xУ‡ t¹y1RTP-"øâü£Í	z|lžØACnPPޏ,á"È·fªóN‡4ܘLßxA'TPkÃØ£ôó¾ÏZù9¬qËü̝xA»Øê* ,zµùšó¼âïÎY¿³TŒøåÑSC	ñ(Ö²~‡ÌdãÄùYŠ¸p'«›¿´Á|_.¹KÊÝw®'1(S+Ê^‰Oë-m|¯¶Âs®év\JTª×ò/¾WÍ÷ùg/æëNìUß
)¤ù"OjŒ\³OÛŠÍ9è(u9q5;»Áõå¶`Gé¶À¦ÚDÐ=RŠrS"ÝoÖqJÞýo+âóÔ:Ä}VR¹B¯ÓܧN¨J@æµ>°ø¤'Æc'æ€
ã
7%ÍÓ<ÍÝáôô>ló;/,ó>w4y|Q.úh©'¦R§lñ×Ùíns° }òKj¾µkúBf›UvÍsxþÊïUMvöÕêa´z·Í2Hþn-´¤ë²à.W·•D!Z©sn¸^Â!ô1î—a¨˜û4Ü)™3oÚ=Ÿö žfÏá·Ãð£Í­rf2u¥¯Š…ÍW9o¡†
ôœ$ßn*§Ô®¤I+v-9Ý&'ç§ËÂݖ 0òÑ_
§©ô"¯¶áÎ`Gz÷įÙ9e!ÀÍÒø"wòö¤+í¬×ìFÌ^MùìIüòF"¬ù4wMüÇk…¹"«[{ɹy½æbœ¼šYó' /Œg¦§óÄ%؂Ýú@åÈaC^5:]»ÏÀ_5X–Š‰ìnËíÄ[M lvš/X¶Æ'»¿³ok™u×yø9Hþy#Ö$ÅÕZ£œ—b+n
"xä@J?/%ÚJ£
ÃOŠÚ÷xJwmÔ:iÿ+aÉ}ÏÐ\jÚ¸ý;±ú+¦ÖA¢X½¤§a€€¥ö™,÷ÇÐó_ö҇ƒP™CVÌ8dŲ‡¬Xn0$§hÐtsì¯Î®ƒïöÄÿ{
·¥È­+zÙk`'5î™û⒝­ñ×p·_/5	ì‹ìØ3ÙmH·ó¿×¬cÏ,q¿¨{ë"Ý,ïì@ƒC"½CW+ÇÁr¯W§Ó¼šd&÷aô·Ö›+žaLG™-öGLº'Ü—–Ã=â$cOÃÔ»"™"ÈǹÀQ™q^	|d!Z^R>2û{õïšUrð¶äL2NŸêº§'åúÈQz¿Q.?i!IÆ߸|ßۏ½ßpïR]Sb<¨"2]©"'š±÷›\¡×i NµÖ5ô]©8åµÀ·n§¤…DI
Š«@'ˆr y¢"%-ä)©lñ×Ù­÷",¾,ð-ñr¹†8m<€q+¹éÈ‹sgìãÖ¨ü^՜Ds¬Á…©‡¹;9ÌGƒ¬;ß0ŠgÃ-íÐ!F¿"CèéYj%"Ó·¤CßíiGQÛõ‰.Þ°uñòÉLÆ£®ôU±°f½‹=T ç$ùvzÐÙ˜1ñìX"V*Ì3[· ÊÓ«çnY4¥ÂP"Ê,TR"pþ‹ªía`uHÊqªÃQdÒ,§)³l^|‹:i–·(™å:m–1ݧÆA0ù{I¹·â6…îiDÜKç£-Ü uІzƒPdÞ¤ŸSOP1΄ַDo₎OV³Gs[ʨ+|OaÉj2꺡ã}‰[7£*Ç.L€í7Éêü)¥†òIæñ×z©wd"2¯ð;þ0h!©³³í?py'î$y‹¡rBñ¶@E·>PÞÆ'ûPŽé´ügg)œ™LAíd3ëmì;c%ͬctoˆ—u_'±c6˜O6qôƒ¼*I¡l]|Î`#-û×5XJ!%
í1Œ´š±¥|9÷Ðb3‡8³ "ó-æÙá± Ì
3SZf¸vqKùΦ•úb~ÈMDÈäqbÿt£€ïòs*añ-vºà0¾7÷dÝA&ãW3úÕªN'e¨yK¬€­H"–=÷A½ü;Ú÷Jêwa'L"ž¬ûŠ8ƒ…§l¬»'#³ñjÙ bZ™up¾g&ënM't£†gˆÆ—gnãÓÓyâRsDVÅËG€¿ŠÓ4¬<•Äh!5žhH
»yñqÿùʈ†ŠfŽ|ñhÀrû»qXï§À¾ƒÖ3I¨…³ECï׫‰ã'†Lë"†=®¾x´ö&Øë
Ã̈́Bw%;ÒÛØÀ÷Áµ	æ€ïÞ"ãŠÈJ7çØʨ<ͪX|¼Æþöjß>º6‡w½FGhslŽ¦bt˜Qoìx"B?f×;Wèuš;n*´ÒICq¢xÀ1âÅ÷ª§lP÷iœ=ö/†2F®å·˜GpêÅ( ,®SÊq¤äO)5Ä·îËmÁnüݽ¡w
Ýü`3ÐÒ}‡†£å6
ÁwžiH'ÐÚ0%ð®ášGC¸*F(7^Ê|"¾Dq3€m*º´"£¥ /Ö#"Ûã"ö{S¬ËF~ ¨£9—•£e.x^oÈÀ8^‡¬ØÉ¡îJÐÉ}¤ŠîJÎâê•Ö›14ýXž	ÎD(Ãl±?HRÆD)öŸÅZ¢xŸ½®¸‹Ét°Ø2àð/å¾åš£ø*€CÔ}~‹ý™ø,
P` Þ ÌéK±ÿ"«oÈR_³Éñ¯N^k¦¿ÛÁÃ…ü}S¦š£MÜ]Ε´ÝËÌd<ê*'qÄ¡"J›'¹/•éF)¹p't_.ð/×°Án¿Y2â!ëwÙ>™ú¢íà©OŸ¾?ø€_jh!_ò[rä‹×Ï
Ÿ^n?úôÞóƒO½u|ñΏøWþ²äKÖGǙtvŠÄèÖ«µ)m&Œþ~	$Q¡ÖÆ*Ž
AЊô•Ê+Š0¢¨rÿÿÝ݄ìnØ[L¿df}.繝s<!×3côWáúðôÇ÷ëÅâ{ÚÊ;W¯ß	]©ÃU±H«.[›D¹¿Ðv­}èÒÌLgäñÓ8h¼çË/¿­a¦=Áý'œÂº ·årËtªÕžö¹NíÚÙÁ
Ç遞ùpŽú`'Ón7N»O§^úß©ç-º¡S9…Æw{X×çëÞÆ©÷‡ø'tZþ™!á½=mN_CÇN÷ŽþÜý ؅x÷ô×îŒí´Üíòjµ7;âmþàÇz›ãô@ÏN
!Ïé@àÔ³]Š[Ò¹.–o
ë4ÝÓîxðæ"NSY*×K#RU8®ûÈ=ú+(ďõ‹Ò»}"Þ…wŸ÷R»9N+X\¬û",q:aȈ¢#GüwΊT,ªKªÍ¸€–Á¶ŒwÀVÎñ^ºS¡RU¹×0—–1£ØÅńEyÐ'`Ý}‹µêAH§sVHÄS#-c!	v"b·Tû>\Ðü·Äå¿2öÛ2Öè	ؖÊ8µL"ƒS+-.š}œL->N¥°"NÑCOJ.xèá'&¿Žö"!±Ù¸Z?åTóóÙE4C"¿Ws~Ÿ8?À.@Pù$ "!¹Öÿ¬RÙØ Ûÿj^ì׫rO	'$*'ÔfdHÏù)ôÒ¦_77++5؞ª,yzÁÊÑk\R
ßÍ*¾ &ï€Ð[Õ¦Œ"£ÏàþºÚá¦ædŽšW<ž¬œZO—«#è^(JÄÿyÇ@Y±·¨8œ@ý&t'wN*X)£VÞ û',Ӊכ+ÅM%&2µ<A*UjÐÔyþ!b
ïd¹±@ÉlH°4'"vÅÌ9öE–Ö²éÕÝúËÊKó3
:Ðúš¼ABW`Á
«ŒšÖ€—þ"•å;µG«»ÂVdCg‡×u‰›$œ—éÞñ6a "ªßě"C*£‰¡©r÷+èd°aM5$èÅ£‡‹"7a˜rÖ?Ÿ®dd»¾,AèOkô"P¯QzÃZ®ŒúzQÍ8Fp^ð…ä5ÒxŒë7$€*²ïÉ äԞªÚ÷ÔT~–žN¾eU뷙XýÄÍ;90&¥KʝÕ)ȸecRαâ¿D¬ôïs'!œÓ Ñr¨í±òMüV7gP,!šù"ä̫½I1ìuÈo½XÌÓg°"‰¡SM^)Û_dßšî¢tºßê¥ÇõYS =ÃO¨+ËSöt¯*ÒéÞpgžC¦^¥&N–!ƒå$´©3Á"£˜Ø£ñ¨"¬B^g*»/!¥a2ÊÒÙ}_:®XWrá(2f]>!•§R¬J9Ì&TVH(••'RTB÷س»ÄÐǤb]H))y*i|‰ ¡'ȋØã¥Â¶ ÙEË4™ð?.W:]¨']\ŠØE,59¾T`j8UÜÛk¥Žð§R€Óïèÿd€ê–"_ªA	CâÛ@Wªe¿µnü'mI¥2ÎJ!m¦â†àt ¾a¸ŠÈÉ|›hEԈ*¢Ð;Âî¾Å֕NÆÕt¥áëJ6bïTǟJ糔¼Rl\5‰CŸ ÇÄðƒÔŠf'Ôƒ…É9•Î×áo§†>ž7ót'úÍmnVA.þgÔ'+ÞÀW<~B˜½7ìWs~/è[îh[rÊÔXӇÜa0X%`¾("›X·måL‰Fg¸"££³¯y9×&ìUÜÖ
²>óᜈ¶r—M`
ú:ccçÞê8gTvÖÂfhFI÷ö0a4¹€‰H÷¬I"nN‹oH7—rú¸·–BA%©EN'Z*«Ô¡îmšfÞñ7Е°æNò"N¼îŒÕ91õ5;kFo¥âàRƒ×µ)†Ø|UêäÈü²ø/ŒÛBON¾Õ3ãMV÷?#‡ŽÔbÜSNJÖ
ú{ª•›ŸSËshy.ÞbފMœ_¾³²~[ˆø&Œëx•¸ÇÞÂáS뱯õñ¾Ktd|+aeT_ÑNœ"ÇS¯ÈΧ&pË
°Ô¼0íÀÆ֝Œmتp[òŒÑTӍGVäîÁßòâÉI×Ýúcè¥
öŽG|.DŒ!ƒßmq~hlWi™·‹åÏ¥¼.¤ÈÖà"6åüöbªþEæ"L+ÌjoRcM<X§âMë"ø»XL'Å#0·Æ*Vµ@žƒ¦ŠÍ«Ä³ß™Æâïl•×Ð^:­wÏÆ5aõíT—žØJJɃÆNJäíÐcX"íäά vÌC0 'VnTpÝ܆÷5§Âå!÷ÚCðC¡~á_ª
endstream
endobj
16 0 obj
<</Filter[/FlateDecode]/Length 14967>>stream
H‰¬WëBÚÌ}'<—$\"À¶`K"Š"|b=R¼ÿ™B23Ì$áÏØ"®}ßkíìÏN>/}šeÝ]®
‹Èóm¼ØŸ&SÉìM&»ûm)ù:«ÈðQàӍ_×I>
"£¬™6ÛñÂie^ÈÕýxaž»ÿ­ý˯ž
©gåæb÷ÛÞuª>Þ¨iõ¼­¥ÕbêZ‰ 0&T1b4%ÙìI'­g2¨@°¨˜Þlq¡¤ÎSTA`D&ܱÒowâ…Úp')öoÛvv2øo†l=µ¦/ŸÄºp	…V&ÝRêE]j¶Ë_ÀqPôXé­J¡+þqŒ³æËPÎ$¬ÖŽÊî
ÐcÛdâhíÏmæ™(¬ô'×Àڙ%ñÁ
‹èυý7ª>	Öâp"~gÉ™[K×É	ÁŽuQ—Aç}_pÚk´ô_*fPý=¨ïL¡&ßõ<ÊIãT–"ÿå5ôX1×
;z0ÂÚu2sìZUy`Yw¿¶Ïì:¡ ¼[="uEä{öµ©ûàÄ|ýŽP •ƒpúŸÞH²'ÎpqpT°"A#;c'
âí´rª?[÷'VOïP-A]Ö5NÁÚi¢ð•¹Søäëgü̟¡QCfŸ7†`ž®5jÁg=wێ!5"¶lÇ+—1ÔJ‹Àp‹óR9€±Ô¹,vÕѵž®ÙϽ{*Ñi€ä¶ÇB°7¬pÀ^CÞ­b5.ò+ökj°§€Í¦2$'±b¾Óöæýñ&¶«e~ÉY¨ãUj6÷¼yßãpR>'`1-£#',—ì
c;VáP #ØÉÊj],ù…ÚԄ_éRVÀ§ÏêÄpá0mØô£y•YØÒày㪼´ø*p…ËÈåDšËÎ*@Œ6'W}§¦£8A¢½â@éܺ°‡M©éžð±À²Ÿ\¿2á³fÓ00
SN|`M0ûޛÔrœÛB1æS'á"]IïÂ9@—èŽó¦šœé-œ¶?˜ö¬
´ÌÕ*½Kr+åÀI#7h¯o·ð¹ÄÿK4Z¥[†Ï]"ÓʅíÒ)TƬWAÈH'ñóî·×•©Ë+Ç(ìäPFØxO$Íõl0Ï9M¶|¨©äù`³Zý*ÀÞËOÛ^&0
¶nÐXmž'xoF•Ÿé¿|-`F¿…B½Å¿{¶Ñìðר¬¾éäýB˜MU_~ßp*zcüÏè3n4{vŒJ²ùãwé‹õYQBŽQ3ô:s`†Joa~·#­ý#ŒF‡ŽÑí	>Os¦ª¹ÔoŽÑo¡p÷=ýÈ2*É0Ön¬ Áf–o´¦=õ¹FÕYäû+2jq%ÑJ"›Ñ–Ê5º2{…˨$#³‹‡"[¢ª³ÜÎ<ú—UˆhùÏó»È÷7ïø†á|ó[hùh®<O_­¾³h²bý¢D§½až"ïˆ<ñí\ݬøe÷|r´*ì±x;' 
¹zømÇñ÷'›÷¯R!n®À[«J(¥úS£¸§"Ð3T ½GvÝWHÍK»$ùp
^— ÔÂVùð$âäßü nU"wƒ"ü(]ðYÄh'׫Wž¢Ü<9Ìî^:«.ü<A™ûÅ<áòtãžW6ŸGl¥ÄoÔìmÖg¹"xßg?¥fæüÎW|øÅGôÁÙɑ⃺Ûu^Ē]Jº»$ùpªœ¸?μœé\§,o¬¥ËZW°‰£ûËê0òQN	:_ó¾Åž¢
j/¶¶jkw뾝‰Œ£~ÀûfEOwZì×Ô`†Vԛ-bÃ0oVÐNBâ<5»N(¨jð~ae¹výŠÝ•†3½»Œ}% mA²
ç
ª5I¦ú'(S%é+1œ´ŒW`ãj1ЉDžÕ÷[àA>é‹=2M/ÝcÝ0"ªýÞô¢ã
<–=ýÃ)'ì1Ì©LP¤ð±†ïZU™5Ûز"w2}ö9žå—ìFÉJ—þäì µÚ|š$£v:âxÆ,¹¸»dæ?`éݗ—ÀßöVz0²§"©!åÆYúW]ËMÜ×U]"1ôõ皻rs¯/þåù
Åø¶X®D²¦÷dÙdTFےëT.èBjžjWJÀâkˆçԅ-&eÚ÷¥4Þ¨îtê—)öoÛ¾ê'ɼ
®levp3¬hÞ?L•Þª,(Iþ˜ïŽwɘ>	«õceŒÜµ'íÀŒ¥6¥&Û/eÕµ7ÿž>Ôöõáßú!Ç,Ø0»¡ªÓú¯"Ù_瞞ØTzBÌs—®> Å¬³ÆÞ/Ø`ÿ­»$Ý?ð±ê—ýd×o]")®t9xŠè
eÇBCLÏ岫4{ՁV!/L¤ù}¹Öÿ¤¢"1v*
ÆüSI,Ÿ"Ú¤RLÇK>òGüö›f¢v]öʊ´'}(—ZÙ©ÇpmÒcGEª§b¤²¢ÕӃùwMU
›}Zð‡¡1~"bWëÛ¥çæ'çö»D+ƒ›1_ZàíÒ}eHâKäIxâQž¸{ìíÒS æ‰8LÁ컪B·Ð*k®œ \²êâæÔp!*T¹.ÁƒN©ŸÀ¥Êr	Xñ'®ˆàº"ÍéԌž_G;o½Ù_Ûä•{¾v®Ümõzcã~RŠ]¹ï
Rf+Ý֚ŠÃÔ̈́ó'0¤6òÄ£fÆp›X@öZKáI'­ÇâÔ(7´Lø¬Ù'±°®[áв×Ðdø(úÑ庒šMÆ=Ϩ¢
ŠŠÝ• â'LÎï—Ê-3î2¤f×	…''ÀÊh)nZ¶‰¡¨œ™Èç–Ëù%7;äÌr;™ÐNŠHÁžÜì‹&)Ø3Äó–ìvvš´`lB)óÙk"òz¬pk…ÙÅÞw•äv-­w[ÂMPˆfK 4Ivéô|'êšw6k'; C·5Ÿ™ó;÷€$ÏÑÍw¬5ëkp%J>=FbHš$Ò"9•yª^—râÞÿôîÔø6Ö"ܑ*¥ágÍÀ%:J
n¾8wx­@SÙ¦¶•dÝ/†¶},¿õ>¡[9m±U°Ç.C|wXÁ|ë‡öXf1ÂEÙñ‹Nì‹Þ`W‰%*BV¾"s"àÃ$€÷'Áu–ðFBaRs»Ç¢ûÌ7¸E·šËä_jƒ[¤ù£ð _œe†iþ=îâ¦òYI'Eº>È(ä}¡š<BìߎðYþÓ],GÊ÷…$s&¾ÿy0«@zۚÕ?TI@0å!Ñ)Œ®U•–>Âìƒ|ß"ƒÚ¯
fÅNß½ú4Š]}g¸8FT–ˆ·Yì«8äWnj¶î%QûHÜ5tEì,E¾2w
Ÿ|ýŒŸï(–­ä¡ê#ÇÐbô£²{é1¤†Ð¾,@!Ãu™b5;ÒÉ~Ç€	M±ÇxcÀ<îEÊÙ…Vãƒ>k)IÇç²®W"søö1ô`1oþ:(´°gn65ýƒYPY­‹µŒo{Wv	-ÜŸ."F[Æh^e¶×$Ø5ßcw¢2G'½…ÎÝÁ2N¥¦7[ž.£e¦Ø¿mSÙ¶÷˜è¦Òƒ'¶ËÂûÖeG•Þª‡íMˆboß-#gVëÞlo1>y ¦q­±t2F-ù%«`°úp@^ʉ{|ë>5Š»Â_ut­§kèÃñŠBd|z"1Qݯù{8‹܍§2á‹IBš£`ÙÉDA'ua‰ƒ(ýƒ[ö°)5½š>Xö"ëW&|ÖlyO%Gíûv¬»Ô²/~¤rvàñ,Ÿ÷‰Žð†Ð%~G@Þ÷"†"0L—ÃJ'ÏM.¥K²€4ܕvjºC|ÐÓËdä!Œ¥Îá|ÀçÞ#•¥Á<è¡ÇB°7¬pÀ–aŒ9OwëYì×Ôà€­t¢†ƋùÎÿi¯òþâ•(ü	|ˆ '"Lb©]I,µSÕÍV"R$øþ÷ÌHÐÖÛ·í½÷ŸüfÉ̙³=Ï9•¿±fïÿ‰‰'ÑdØ¿!ŒüËþ@¹ ÿåف«‹¿ÒÃáQ@7w߈ˆKä\ù‰&»Ï5¬ý™,^ðgÏ<˜àTàéM'‡{rçæ¸I|ð‡k-;4?¦ði-©¬ÇÞÅӆ\–‰ܯñ…A=wJûs¿ØÕ¹	îÞ£YHŸUβ'\eébìOr¦™iÎ%~—*ÉBì¶%2§J~	òÛHmׇ&E?²ŠçQL¯0£'éW™MfŒ8›J6ïØö|±FšöÊ#í5@úuCä××ó2Ê7âT.Vû¨ü6}Aµåd†Z•Pµ‹óºÙΦ¨ƒvKÔé¥÷è6Ðñ¢{îƇžFÎêõºSÔo†vhê2hPñ6LÓÔxsû¸Nš{aÕqÐæ¾ón™+.	š;ÓwL`>.Ô
ÕøTê<Ý¿P~Ý­»cÉ¥B×[ù'g¶ Î8_õº–Ït1÷ÔF¯]5å휚¹P{n®ˆKÀQèø(Yo·i䞌aµ¾¾ˆ!–_Ê[xÃvKq³×2Pîˆï.®¿¤›Ñ›\&"Æ"¦‹å‰0˜co Aªç3Íj€=éúIÓ°¯Ë¦BŒ"tåZAúô¹"òµêÛÖՋŽ'¡rœ²äeMǪˆ×ûXÌß5Ö¹ê›Û—'ñµ	÷¡ØzŸ>žwæ};"&^;SíÄ>GÞ'–Øy(_ª¦<Ó¡ 1Q)ö9X£ÜjLÇ#bNJ»—ÿ•)¿áM‡F̊éôzvYŒ›nÁŸ':7òÖ«/%˔Iœ£kb%£ÖFà^^20êhRz¿pÉé;þ¶CÈäɃ¢×½Nüp¢à;ț2Kò¥ÀZ	oOÖ´¶®ØiÏ#ŽøHÉoëòV¾¾½}ØÅ­gf®|§
¢½')g[Cw.moå§
Q¹¿ÉÚEþ´µ×‹loԄãFF/ŸOûÉHÁ«ç²ó9îôû¹ä|1öæü@e,Üãò‰OÛ×=l4€"| "½¡`Z—üÇú¤DÄÞ¯ë>ã‡*{¢4ÁP4-Çàt
\[¯ÈŽ/Lorâà¾þâ+­EζÁø®"ï²  ø†ø»ràÌb[ʽ¨ü0åI¼¬˜=¥…_Ï ó¨ùnã¼qµ»W›{Ëq21ìýÿâFUÉ}¥X#Ëë3i«Åqš²úJЫ+ØñÛY•£÷º·P,Š¾eße…×Ý0|T|x^£Z›ˆ£^­`zÃ[a?ê"aT.ú°_F¡êåG=1/Šk
Cöh&WX®]4ɍBß0íòÖÙŲG½S´€?˙cV.Æ¡³­êë}ßõ8¨´¥Ëâ-Jp%¤ÄB±ä¤ç›æfQ½¦,c®6¯hå¾¾_Ú=("? ãWXå01à®<
}¶'e×CB^¼0
öh,žþ'n'~»×ð‡×€.³È®£û}™äU'à¬èƒ
?/d•ã2ôæT"(¢rÇj'öýĽÙ+ÆA'<k1¬Ý*Fxدʅès‡Òu¢P†5¥\Ú­z¯Oºªk¼×ô¸«e"³çy¸ÅXð(Ç'³V׸è -—u%-ÂçκçŠ[ǂ‡Î'ä4LÃ>œ®>È5	O¬ú`|-p¬Öé°)¡êSº"Wƒ¤7'k <Åçò½à=ÞàßÁÇzº€H팧žão\{ÙÌ.cZ
ÐL¾ö¸½±žœ'êx-‡F¢Èè:‹ž²Ià69¤–Rkô-KY+2¡³4¬²$ã威9 zà!¿Iðx
Ÿ«N!7XÈÊñ–åén'Rïkˉi¨`<£VpDòµ‰5Jùª÷qLþ('êÕÃ7Aq^ÓiS,äÞoQ9"ÁŸ1ÅUº
ŠŽâ¨ƒÃ¢sFù¤UšÔÓ,âÓw4ÆnìxÝ8R~2"mï$m8ÐÒÊàR‡iÞ&·"¯^µø-É­½×)¥²zðXLäZRVò3zͽo¾-#Œî1AbאÖóNïs—\{I•å¶v«ÓƶIÒkK=1*Ó+Õ4Ó÷.R҉ês-û
ÉàýϲêÔ³q%B9uª?÷ îʄûZáe#Žd«²a jëT®CŠ³-px#ò¹cmՕR«KOº‰~$™èòÿX²~W²øÜ÷KÉÇY_
6fnš^.™ÜAÿÑè!Ù¤Ô_ºû×1–¹éû5›'·»‡r'ùk¨)"¥7¾[1¸€dOXJàßAG]‰rSJh"¹²ðzZ¡>$Cæeµø6ßêêRP¬\«óSóä·Kž¾dm'c¿¶÷'kg
\ø;ÙÌÞC·»×oªþKÅ´­úÿhú/ªg"Ïy'34_uj—aВ,øWŠâŒ
éKʸ/¹†€‰Á³Eq>	°Ö¯pT èQ¾ù uÕxÄgþ9‹Ÿä~WœÛûåHöÁüò# mg"u®ÓE½¿kSÚ Z›}#øp_‰"ý—Žÿ¦ºc—þ}È]P×AÿQahuðjlϦ›ÑåÙÒ¿"hù'˜uÜêg˜ù›â_ÅØoaæ3¨ãþ姰þs·cì',þ
Bù`wý¿-Ôý"ÆþCþtÐßPø¯¦0_Kvü{'_Ì«c¿¨Ös	W6°ß1 ‡FY³«öRöd»œD"ôqwU™Û I~nTu5ËFJ2·N0н힠·¿HÓö&©™O£Zd9ê¹Õý°^"xsçVU±Ý]$£ÇÝÍqî©ä*$÷/N	†ÍŽÈdýù÷Ÿ÷ ½_æÝ8ãA¡ºçMd2N•ðþ Æf¢®­ÆÎïgr»sk&'qsúS³+£Ð,kÃ!ÔîÇαü™èõS×"´°BñÎ璡¶¼ ۖìvC%a<b€ùs½Çï•Û*<dš:	ŵå_¶…ÞŠj0˜ºD¤diÑü‡÷*ÛNX¢_À?TeP㌊šhLŒ&ŽqˆfÒ8»Ö}ºß~«[ô=`Ì}q5´TwíÚµ«Êì¡ýý&Âjãh¢{_Ž4Žç*ee¶vkݓo³h#ŽŠ÷yªØùŠ(A§8®r˜cg莗o4%YUXëE ,|àÞ0šÍ¯¾fÉ~`J²ˆüþñÍ=Ÿñ)g¯*9),7o´4‹•‰?@—Ý.YLÕë=ÁQÓpsù÷@¸}_Añ¸NÀO4eâò?F£îUêG¶…籐àVñ[ˆ~Î_õ@Áyz"¼¶OÓáôåàšÿ•úr²àþm\ݓ[|ʹÇÕ?N†)é©ŸÉrj䘴Ҟ€ci¢°'/ÛÒúÿ­/šÃ?ªl;îÔq‡AafW†"«v\ë'Ck-È ëî‰;8Þ©lÿrü_‹Ü^¥[él66]ñÎOl¡Êz}µž\(úÒëD¶ԏÛÛÊRz˜\ûçQ"q̒šL®ÓtÌjrǬ¤×‰ÉEPÖ'iæÔ©ï¥wË»¸é.ðglº,'nÎqG2
'ô0$3ö)$ÛÜ 'ýøj"Ì«ölÒt—Hºû$Ù§—úŸ—t߄ê$íJ±h÷…¤?Çéž<´Ðg<ÉH£8'åŠIM—wødýsôuGšøXãòÏîÂrKg¢¡C³ØŸgÿôäý¶
u°G«ùûMLªÇ{˜Ëe†ùl|$+OÏÓZc²‹Fš|¾ŽòÐCœ<JX™¡êøužI† Ì
®±òOx݅IÎÿädâwF‰½ãQô!Ù÷Æ'˜^Ìo3ØšCR9s;x×=S^"1¥~—dg|"ùúp§¤ãŒÿ&ÉNf¥÷Õð@ÑÙց3Î*Z–;œò'Ù¤q'ƒÂü;Å7å
­˜èçõ3ò4ãZoe–çZ\0ÓÇp%ÚC"Ú6ÇvÐêû¹Y±?Bu-"Á+‡c¯Î"ûw¡—]­d¥úõbª¯Á+¥CÂ*ÂoQ¬–Os𫟱̶¤Ò]JrÜû:žajw×`‡Q–d¬=äâ¹ÞÜsRm¼©îâǁǁ/¿xs½åOÃNP¿xv'úåÀã°Ô/‡¢ÿ»Ça‡úò»Ça?¡¾X¼šû¯¶ö«8³)·²Û%óGSÖaŒP–´ëˆí—V;%íCafüprù–>¶¬3ÿþ¡=:0R(wõ¥×8&ö˜¨L†ÆøÕn<
×Òèí³Þ¼Šr¥ïÓ/Šß]ί×E­³îRûÖýû¹NW˜_ì
ñÆàîLÉXý{;ŸV7±Tïc^¿7´±vÿTÙ7àÍ7uP÷±	½¼Á¥À˜ Æ8Dú;à¹ÒÐ)d_ÞyÄZ}כ»Ôw##¶—}?"yªå'·ÏÏ}@Âö´¹rÝ
˜ÚŽWâÙÕô€
d›ÿ~Š7hg¼96¤ÅÀÎ:Õč|—šµ5xJ·
WïP7^ÚÐV}˜¢SKœrðϖY,Rõæ6+?œý«rKèÙ|Y¸°«Iž©†ØšÄˆ…È
˜¾eÓ®e]C—ú}Œäë‹S
'"×%»>N‡€ Ð}F:HX"ôòqB˺YÚBPۅ€ýˆÉ; xN§
B/^Ú!¼ÔÔds(iÉ1JM/áf©²?EßnAȵ=¶¯ª	 éáUJ#q-` ÷7Ǿ–Š‡xàØ(ìæÞâûÃß©tÌb²ÎƓL ZB7¾7'iI.qØ@ϖe4ÄNsÃHÈcg¥ªoÝý7êx4ÄNsÃ{qIµgåË_Låå¿ïà4²24Ùrv;¬4'šòoMyyŠÂ8¬Ôl3
'æå_îÐ>t‡º6¿lMè¼<xx4ÑL¸öq0²r‡Rå7ã†ÎKë¬DÑ:/ q$7œ:+ù\ú±¯¨Oö£uúñJ%µ½m½½k'6ű¯ö9F›Ð¾£È҇9f–¦´Î1KéjD̬ötÃȱ(w9vÌ
cÖUgÃ1úÇLCiª""ŽtëA5!._vM¸ö´Ïò\Ɗ|‰ãw0¡|¨"»…'—§0Âe¬È§	—ëôŠŒG®áאSG³Xݧ7ï¯ÈpÃô•à'…ˆüÙãÔðu'¹Àݚ'‹A<¢
ìû»"‡K8exï±£éÀƒ¿¶}¯xÞéáð#?ìuœêêkè'orôæ¼7ÇÍ»9F};QO˜s«Ÿjà­^Tæu4ñœ?Ï'¿§…%?Ú|®·
©•´¾aô@Š1†Þ•Ó6d·¾!¦Õ8Ai[yNßò^EޓÚFIØn¼à™•ç²1—þÎxrVf
ۓQ\²y¢³¢Å Ü@yþµ†²€(âöÆ«$<Þ'tÛøÂʽ¢/‡)Ü1sŸ±~uAø¶´€¿" ÷ÝY8`~/ªþfî¾é劏#4¡TþËè%Úeàõ'LW;¥¿n¸Ó\/j¿OU%šñ}ÔҎ')"­=€1ÚÁ©¥Ñ`ð€n'›MäƒvŽ[!(ݎèliÍ}|³JÂ1¬¤óƒ©»^4®VD&ÍRkřËçEzܹT‰Tïù¶Nö0'¶Ñï—Ü@ö«œJñ~ú…<
«¦Àßø)ˆdÿE"Byû¸~Ï«­>l@
⨌í¹Þ0ÊnTãÔ¯GM^[½èÌꋎxARo3x
/¤·£tèæ­Ø-ε¤}_ãé͛
zƒ'áý¾|\+¥Ô8xD°Šjž+ë1?p4åCúºƒ4££3ÀUͳ=ôU¥Åê…²BÂ	«ž€WȗÕ@Ôÿ	ÒTžÃ»/ßÞ}äÿêIqÑR$ð䶕n'
mc؋¾ŠH¬¾Ñ
`r¦•ÄÝ3ȇ"¡°©ê͑hÔà†ÝÌéÇÎJ‹~ÎÁH+iŽ¤‡Q¥çÞþm"žúԃkA‰ŽÙÆØòo²‡Å2+¶×Ñ<÷Y[am³sŸl˜'fÎAD!s³¹Ãög³º»ÝƒmTá"À!¶§T˜c RڕoY,€[/·#žrrw"`'Ò"¨ÀóþþmýEÐ).dSók''p¿—`ëεõ5e­¤_¦Í»ž-?ÛÈ!èW¾RcÛDrnE@Œ¶sñ²ð"ÉÿJD .'¾`è'+¯ÇÃEiñùþ9¹`‰Á%ó'P¦Êb8¬ÿ³JO_×ßÃÉê"|Á%å|>èO_§ƒ!ü´«"€U免ֻÝxØ®ðFµ%©ô[(;Ê]–c½ô_—dÇ%–öæb¤›s"	Šd¤Q"¤ï!'ýø"­î›‡dÖáG'-ÖÒ¤›/Š˜tª‡r.‹Xau:_7®¿QwW™ž½ü@ßås¡ŒzT)ÖO²³»›Ämh)sÑg2møž2‹VƒO7"zE‰%cÿc½J»Wšð/à?L d\Ù7Ù'2¬˜sçËýíoõ'Ð0Èxõ=žÓ©¦ººê©§ª†8ðôŸó	Õæ2&¸®K/äng †ülØÅz'ŒÏÙ½×b×î®Æ/í¢–IÚE!–²‹ÝQžÙçûr¨C8dlEßÄîîç»b…cnãHÔûÎù+¡œ‹Ûf§$ऋɗÍ#=¯ZÊf~¢¼£o<aݘââï¦å]uˆh‰£?$%÷œdýPö¤ë²ç'j•0ïç™`ÄóASt3y•îæ §0¥ž!×HFbím'¶K/¦`ŽÏñ %°'gc¤Å€Sp©gÎÎfvµ´¬AuÎLúÏT¥=´,gkf9¶¯)%=¸S¢(Ýy!»)Þ¶nš*¥'DªýÅmÀeYAcƒ
Z6ˆZȗéÑ4Á)	´¨5ïp$=lçÒ,Jô–Âÿ^PùpWPšeù˜>÷u5…ÉÊÚm0¯¹B½äÛU~¯ÆϤ]H´Ü@2Ư0lLÌn¶ê³àÕcã;(ˆL_@*ß ,'† ýšÈ[ßQ'M¸¼'§Àð³/‡È¾‰ë~£¡Œ¤ =ã´&¡6O…¨]_`Uã¼l:íkLñßëQ§c¿Y2^Ö]Ðsdrï³.þè³ÈÃÅv\a›–ŒlDh‹»É[úõÞCÞ»7cþ¦%šžô5—/óÜ,õƒ3ª6.Ž6üñ|C9gY×/–Ù_)3L…¤$úhè 	Ð/'è[ï>Š™X'@.rÉ%·À´z#u>Ú¦Ácíûó\zÝ
w³At™^·ëù̍³¦Ç‡O½Bú9ñ^É›D!òîœÌ35%3+¥£û9ÍY€™'úŽ{ނ«Xýuõ"Ež!E‹ÇpCŒÊãY·P}Wؕ ±â§3O7'ž˜õ÷šˆ^Ð)b}m¶Wt¦ƒ©E
µDЉ½RŠ¶H Šo2j¦¼‹7ÔåÑ|jšÜ¦KÈFñʔtbçJ7³)¯ìº"¶DzÀmøæZ%¾ËÖøk¦K¡-OvìG5àQ"˜3&§îÃK%f]v#l	üh"gE1sþ4ãW'ŠLK+*²H~€sÉÏ÷ W0Ök͈AÁ¼Þ'Âë
,3è""SŒɸ~VÞ º¯uØþ#¼¯B`Uˆ"ô
OÒMc»0t5þ¦éÛµø›Ã‰f•·H¡Sn—"ôw=‡áÈd¸
EwäF)NT€'	¿—MРÀ—§_CP_|®P¡)QÍvp'ü ãoP÷ëùÖ6º>q""º›=ÏCæàû…µñ´UízíÚ¨q`Ä%4,>(rQw QsÏw"Ÿñoîس»©âH¯·½[¨‡|´…ðéςšeÆ-=Ïb—­k'1ð-Jb;:´çÄÐЬöÈ'ÒÔc	!	»²-9~ÖÀOž*¡á£´´q–=³çÁ{¨RFÅrÂëÎ	žÐ¶U´\ÐØw‡qAkíÀDT'$_FÓ	`ëÄ5à"S.p;D"ïKÂüÔ	Q>µ&N ‡'Аì;ᘠøMer¨ïª8¥.ж*xŒqÂ	È;`7ìK9M\°N4[;ðgùõ`ڂ²Æ3~äÂöÞ1(}¨)N+ Ñ?©Âý]<6î›!ˆŸ°ÁƝ´ÂûÝkHXõØ×®!ÖȗT(ßR îظ/©…ƒì>ÛÀcd·èþO*Ž(ø>Èâ6œ@ yO…÷*öl8t¥t,œˆù÷¢á‹=ñ<Uя÷U|T6X³XOT¾™¢ú¡pî"7DÍTqy¾K.ÑÍ'÷öÉîÝ>çÂ*QA'1×öwBä@NÝJ>dÆ>ëù#€œéÆä£ùé*ÎÊO_Cùbºî0&«ß½†ö¡
{;'ñ²ïï6äü·IQ°Ž|Yû¨NÙ ‰§m õåc+Š/€j_´W'¿'ñÚgšèÆO—öU։¬øQ²˜Ú½ÎÊ×8;öfŸy2ìÄt'¦ÃWQ_Ðù´1õjÝÜHTäþ»Ow0¼ái'Ìq¾hÍ!a¥8ú.¿ÃÙ*ôè¿€—ÐLƖ°zðFŽò;,c^²lºˆß|Îp¸—é
­<šmÇÖüɘ	w•EϹÙ7É
,È
jêÈH¬`|ûƒ™rÙS¼Î»7Sô(жàè[ß<Œš†–ÀË
VAÄGC$ õ˒k®æ."ù5¢{Ðá,ÝO²i°R'Ÿ¼VÇìÔ."|}"È–áeáIÁí¼:Ìñ'*¾´ ÷½$ÁLÐÌxä‡Ê¥xUÄrM¸ZŽ©JäEp^+ڬ¥Å¡)u'FŽ‰J~sG¥Ê»è­àa#ÿ<I¯»ì7|Î'¤QþŽÆ#úÄü–FU>7žZh}©ùãWíá®	/;Åo³¥Åç˂Ï??÷vð҄íhj^ü™Š–ÊݒÜ&øÖR/w*~jXзYM£oÛV٘ÔÒB¿Kß´q)ݗ*P/ðhK­;+(ø·6NënËTwOhXh{Ñ{z¡ÑOKà÷¤ëºË€¹KïٞD]È­nʉ™4vÇKÃ…TþÎ^ÁYy%¹?r‰¼'±4'èP—õàУŒ™;ÐÇmïtóжLòÜ¥ÕüØVŸ+Ô
зT'÷aµ}tg}?´§˜¬¶3©™c/W_/ÒoìٌêÃÂÄ7C8¸Àº±®/)fæ"`zUî‡XÉCܖhtEž:$yâ(¹` o…—ý€t[š^¸¸‰éÔ"©9çÏèΉ–ga²€ßÔQÖæ$䬨}G'¸Pž¿ Œ	Ëwԁ PŽ¸·L(,²‰¼ï¸{ا)׊š‰a*ä)GFîd%0ÈGÿ ®URI݇—
l)ªÄ;$Ø('Šœ½uÑ]¡ÌÁñE×ð¦"´¶
ʔ¤®ê¹doׁ"GàÙl™Ñ
Toß"Oþå¿[ÈÆÅïTµ›^Œªú?›Ôr¸ë‹ãàKEßlWhC ›ÐǓE¡ÿ[_ÛÔ3ò§Àz^ݜ©Úõ™À"€¾6Þø5Ö®7ÂYj}WŽ¯7©Ép3Y.úëßgAô©ñPx\Žt¼à+õl·ú61Ò3/œÉ•Íz²ŸñÿÌgØæEE®g"üà¸üW¶¥Ô3ùn±Ùo~¯¨ìY÷‰¡ÝžáÛd6Zëºç¤Á"ÅÔöWzð—¾6`×_-æÉùÁ.Æníÿn7³±¿Ãۍn­ úóâwý÷ÕڛȑEÿ¡¥|ñDq»Þù6ÌV³òf¥ÍLâhµB`›Èv#Àñ8¿~ϽU

h{#m;FúP{Î}Ô­E5žÎð~W­ºÇu—Ç®ãj"ãÚÿu0Uw%'¾Ã¬WŒvY¯¢ º_Îî—"'É];WW󫲞^¦é¤Ã
ëž Èî*Cë,Þ!Ӑãz¹D!>{xxh¨2¿:£!‹Ùp4YœuW™m²ûä¨Cªµõ"rQÝÏG"K(2)ï&˳Ÿ?¬~<åx9îª*kÎûT™/Ÿš#CÆτ:Sê+œ.ï–Ão§w‹ïºªóÜ{KàA"@ÔÉòÙ µóhԚòh>.§¿OFÕímu·H¥¡»®&fûXÛ³žÝÏo˜êxt6IÞâL–ò¬«¼Ç£
`Ï؝¦µ–ê˧ÅÛbÝc,ºl1@ŒŸò|¼{¢x‡÷ÅCï¯/Ýn"÷t3ôR³Éˆ'Æ|¹C#4ž¼šæ}6ø£­Õ'R	xUIü"‡'u¡¹IÔ4¸ÉŠ–Ü7ݭǝå¿Eï@«¾µæÿÊ<ÿíóÇg1—8ñ!^÷ǃÜsüžVóéÕô®µ
Že0¯#¶9>!Ǒn0oÔw¥»Ë}ÜâÀþáÏÛïÉ£ÇÖûªºI¿ö©Ó›Œß?~ºUóåd¾Ó¾éþ`C^ څXœ¼).~Ù×)´Úû`Üz>O.®b	™ufü#pšºñÛئ™V=Jì•5A«Ã†¶ÿ><¼šèz2½º^¶®F͎–ÿÇ䯹ìÖ¹‡éxyýœ¯Ã,3—ÿ©˜.Žô|¨á›ì¾Vóñd>ªnªykšß…¯ôê,Ó
Nû(W³áhºlߨu·1Ùâ³Kx6¼š<Ó×ü×YÊ
F»t¯æHåêf2ލÚ_Á¨	ïn¾Åé	Ò÷SXðÖÝ¥¼Åh—sõõ7´v)Ò;"ܵFGÓcoK+´¡³Ä7Xº`"óŸ[ºEÙ]‡?M숋ëá¸jÝŸ¨×Á¾fu€üUuۚ¶-uÁšW@?ñ:"ëÏhT\)CŒ¶û¬G‡#}\îéþyz7].Zóïðc/µCž¿ŸÏiäÍðqÒ¾ãÑÝmY÷±; ÃâºzxAí»ÞtùN¶Ý!¦wršï«m‹'Œ¯àìߤv\ƒëÉôêzÙ¾RîÕhPS;.Bû.0¼'"pMê8ógœ‰þõxþÉC'êÝÿ"uoMç‡ccøóvýéç¿
>_Oo&tø&\gï«ê&ýڟO†ËÉøýã§ÛY5_6¤/Ÿ>o‹"Á7Ý|.&øòqð¦À²ï>I1x7_bDÞ
ï^,NÞ¿ôîù%ŠöD©²¥RZy|jŒqø"ŒµN㋣?úÉÅ t¤/^ØŠ‹!ÖÀÜBá}ñˆ‡¿ãËo€
)Šÿþ(ƀ/þÕÃE¯;h©J§¬-n{ÆÉ2ª0ã½,΁éR"֘q¦"ÊÇ4ÓÄØDD))ú='"²¦PA•6ʀ¥´w%•Ob4Uç61Yš LAHPºaì®ùýÞe
Ã喿Ž™
—×:H?{¼âsŒ"ŸºFÂ}^8;ìûûž,>ÀKQ*ã
¤÷Ác{òNOM^‰Þwø§Ê`¥ƒ¥"áÒ°Vš¹úRé¨ù'hZf¤ÈÓõ£,µXý^H=½ÏÏÒNqç$˜W,uö;ˆÏùQkÍOô}½Æú‰vH&œ¯€l"E‡w³ùLÉR5øÒÉa¶— eÚÄ5Ä[yï`´ÞD² +LňP´E¥±ø¹gX"nk»	ø-²¾ÄOX3BI¥1¥Q"0ÚI–3#£ž˜¡1Bؒr"±"2õnýäbJáµ
(Ù½Vä~ím`,!œpµJ;â'êßi•Êé—åÀ=eÊþ4ª½_ҋR@#=I‰¤…
€'õf-Ká¢NˆŽEÁEˆwޑǁ+U"K£œ4ižsB1â¹Ì"Ò:gò´\ZÊxØBHŒ:-¤Q؀('I2ê4ya"cLhª~" xØå2}q95êm`˜–ç)›#%ï&u!"ŠÙÊ(QAújø•©h—/L'ÉÊh±1Ö¢Ó(+e^Ý$@;aÒöQF –Ë䴎Ïuße$dz…–vÐ6šÌm…II©I9«81BŒi;…Έ—!ÔZz›ÒÇê(³•.e€ä̀¸`Dy¯3;¯(Y€!µ²´!‡"hm tírɞÓetÈQÙf»€#.Z½F0M!4۔±ó&–ƒõ|7¦Ÿ".ù¸ ›üj•Í	àwÆ8%4W% 1$û¢	‰!Öjˆ RØ'¨ãÌM'¥à"M;vZ³¤yÒG§¨5"i_¯ìå* E.oF&‹'×9úe­jHµ4<MÉ-cQ™4ÊûþP\&íƒÎcÈ?#žg£M9'–zF¢J˜ÚLFÈg˜o`çM,ë{þ"ÈC¼‡U)漺öŽõj1ëRôú>Æ8ê©`%Ñ°>Àtv 'gt^ؔè#d¬Þ'¢MÞAN2n¤!K8턯c\+•±}¯N9­¢Ž›ˆQ8ìR4¬0G`Z]§ý˜›¤e®6f¿ÆZ?álòO&E±"1©b½Vk¤¿éÆ6ü">ÂçÏ9ÏüËÎ3ÁŠ.RH·yD¡—ˆ\)÷ho×9J‰Ñ<ÊC.Z¿5ú[›ê&šP³‰­«
öÐÁ"=æ~þ"Íç-[`åâˤ:î‰+å쁏à–@Ô×|Œ{nu	J g4·#¨ˆÔTáÜGì"	£üˆ
}¹¤¶ǯ	©"£[Œ©ÑËUÛ¸Ô±Q˜òáÈR›GClZ…:P~¦îšv¢Þ'æ41|nf{šârΘ¤+—ÀɍB8ᣢQ¹5>#¨˜G<Ð2†(@â‰Ü°òJ'ú§
Agâ"[ÂÖ ÄÝÕ±íÕÊFá^|µÊmeû‹•FïìIVÖ(ß,`zttu'‰Zp÷ïY;tNª5²¢7ê50ªšt:ÒJî¯'îª(•´]+â¡/y·á–QQÿ
]ˆt>²QÀÙ{™5B‰@'oŒ¢¼N…4¤©'ýÖPS‡ý4"ÍÑÂE¬â^—îÒ96\ãÜY?¯ÈÕ)€öÖ«UX%‰6oµ×JKÚËB^ï8Âp(Ó(X>·
¤"Õø·'í ª[lŽBË¡¥o¬´íº~î"hSA!/àeȧdÂ"à$M­$ݺF0#äŒY#‰¶L{…Y
ŠÀ,¥¥Ö!Ò-QEVM¸â«ßRò<ë.¨ÓÖ!'ˆ§B‹/Á暁Y#‰·¢êÔ堗È+¡šA#©Lڏ{Ñ>_FÑ8¶Ê¹"''«BÂEÙVäjˆNÑ$¬"¨|@%<Þë¿ìWMo7ýþ:ځ³å÷Gz
ŒÞÒöÐ}'×j£Ö'
Y.ìß7C.ɕdÉuU@-Š Éê-w8œyœy£ KR,qvæ+<²DõˆûÅ|Eœ#1ZWÏVŠ%Ž"›U<¡@é'K2L¶RG9œÓˆ«K=Ž†]«4't]àvr€¢{C4 b¶',,¹©
Ù.B$ýB¶£#"ŠòŸ¾Ë=ˆ8)–E$PÅÈÛ Z[×®A	ÐÜpzEÞ"³R2YP	'dL'ɲ§+ùåŒV›SjM6d‰?46moyä¶	¤Éê*G²4×)§}êTǙ-$HÒÍ5Ò³Vs"²bd/¥t-Òԉ'EîˆlG¹"ƒj˜vstáD'Ò}Á¤—ê‹O¡µ"qORºè¤È2µë"
QÉ2k@
£‰\5D*;W;¨D'‡Xm#'SAê†a|DC(BPÜˆbt¼5í**$Å*R)V±bƒ¥JŸa¿–cTœüˆdôÀÚ¼'–"ŽI†6a´Ó¯}nL32…¦×o$r:¢¥Ôº]¥³èšq¿‰qD3`ÂÊÐð)ó‰yÏ*RyV±Ì36äTÃ3ÚSȈg'Ê¿¶…gƒÛ
‡,^3b…€V]Eü´#¦QË5zÄ´-Ný…QÄzÞ­ƒ^ÛâÀïóõjº|¼›®g×ç©A^ÂwŒiúúâbòÍOëÕ|ùë$­ûå~µÈ{&O>¯ñúæi={$»£Whu>ÎøºÖ;—,ՅȚ½}(¯²—6F?‰ñ'>co…h¼ý|{3ûñæ·Y¿þ~
ìyc˜¯ïâ'7¹>G5òYòRПᇥVmÍ%ÈÒ)iþ'¸Æ=Ü)níˆky•Dw!79®ðUûæ°w,ØjPp»îˆ:]£hy֛3"W°NÇì…Ò$Üɐ'Q}AÁªÁ‰§`p½ËvÁw* 0p»V)ƒ»¯[KÒîW±ìÔ`¨ú½uº~ß°ôÃýí,ðó×ùãww³Ål¹nró¼¸[bÙGúg9]äÚ°ûýÓ»§¼@æºÒ¾^—ÒVÓäÇ·uMÿu~w»š-óš½?ÞßÎð÷Óêù ³çþ"Â++·ÕÑÝnNËí+7otŒË=§|ùoœòeï)û·œÒRß5á"OÙ8å«,4"•ê""Ù?lÏò­Ê²Ñbúùª¿›)ïw÷y@Ÿ<IuRX¢óƒ¤Åƒ"1 Xâ•7έyŠjo0!ð6hðŠëE´ÃF€Á÷Œ8‰O´ªÈ>Ã&AøŠ}aLû0ú
Pˑõ!'©AçC""%hM!Ý.ˆÕ9þ'B_½j?¸$v!{G£.1Ö¼OY
äû•Œ.Dʆî"÷²b"8
7¾¨#
BƒÚcÅ,Ba«±)4ûe¤ç¨zþu•ì~µ–
Òì×`Ù«b©x¾y¾ÿû1ëq§™7'[ێюOÿ¿ÇNz¥8é>u¤v¬ƒ=éc³ý¾vüڠی"ÊÇݶsWC«~ٜý>äfÏàÛþöü'¨'C.[ÌNn¾'çªñ\e£KSz)tWh xapÅÓšEäò˜>Ó]ä†m:\|ß²‹&5©ËÂØI1C£F³—Škëx";?l+çXDˆhÓ`©Ã0ûÑÉ
Ò§¦ne»j:ÒÚ	‰^¦í4ö¸âÉVJ«'SÑ%$*D'·Æ™Š¤ÓÁRÖ`Ð::^%…p)JŽõöƒ´BiYþ8Œ.¡
89uMÉfÚ¨¡EÊL"âÊzN;©+†
ø‡ò6â‡ï´ád¢q—´\è²P€o´ìtd¿u¢·-R³9`•Hf;Ê°	K?¬ñÀ¼BŒá˜;DƒÏ«µâ´Dãõ¤œ« =Õª ›UàE!qÅé@œCƤöi;¥8¼`""ôd§Œ°Ä1ÛÃr4âtV¤!kÁ#4sS""'‰8'吝"¼rQ¶!‡çm:6"Féüp¸x$Áiß'8ßT›^±}°6í1þ/Vuóåï="ùiöüp¿Z|¹}˜î–D*(c©O¯[î>ж:Ø\÷|¤ƒÿ)À øÒ
endstream
endobj
17 0 obj
<</Filter[/FlateDecode]/Length 597>>stream
H‰ÌUÝn›0}ÞÁ7HDŒ¡`讨ÒM'ÚuRÛµ•"‡8"ldœ,yûÚ@ÖdMš›F
Q"ûûóùŽ9_ÊÛ0Ç>€#&µªJƧÔÑ?r]÷^˜
AÖàR-¿½Çdó¢œ
Êú˜a'É'3">)E1YHÚt¡ÊU°×&#5½¤«š鬦uÑ×y¾½ù©²Ú"âfEI©.x¯Š²|rçÒe,X1	çù¬W|	‡<[T"É>qñ
}ÏÃ0Ë`¡Rd!×°tš')9kà¤ÈádíÖ,?pԒ"çBÞ;)öÑÜûß?Æó¢¹.©æcÿñÿתּ¨B«Ës"$À8°=ýћÛÂ؍'ÀŽ\?D~Lü2ØbM
šÕˆô6}؎ëÝ _†ÇÑ\+÷#oTD:BÞ8RÙû«Þ žëµÏö¢Å聤¯¶ÊØ^u¶€¦S>¡w"?4"·mÃ=*õ5T)ð<5"`
Àó"ñØ]¬<BÜ'Dâ@?~Ï$b/	m»qŒý‹0 Nh#¤Ûè°¢ø$œItÔá^R;¸ÀéL8ê†T-§;áÃû{d/úrñ˜`%™Ðòøܺ!k*:ã©Ó7òÉ°Î_ԕ²o·Ôížq³[­œj¸¶Z.‰¤/–ï&!Æ(ô©s¡æj«ÿÓH¿åÐ>Ú#ù~±ëò"8_¡ý›+ÃLGáøšM[8Žaš¿HNQÿnÂȲ¤€0Æ¥bªVÚH.(hæü¯¶¨"M¸i^ß}7Þg¢Ò
endstream
endobj
18 0 obj
<</CreationDate(D:20120919101741+02'00')/Creator(Adobe Illustrator CS5)/ModDate(D:20120919101741+02'00')/Producer(Adobe PDF library 9.90)/Title(CC-BY_icon)>>
endobj
xref
0 19
0000000000 65535 f
0000000016 00000 n
0000000076 00000 n
0000014971 00000 n
0000000000 00000 f
0000015022 00000 n
0000015438 00000 n
0000018351 00000 n
0000018239 00000 n
0000017513 00000 n
0000017678 00000 n
0000017726 00000 n
0000018424 00000 n
0000018631 00000 n
0000019624 00000 n
0000030493 00000 n
0000043468 00000 n
0000058508 00000 n
0000059176 00000 n
trailer
<</Size 19/Root 1 0 R/Info 18 0 R/ID[<35B887E2F3B84963ABCAF314AD20DA4F><BCC3CB619C3F4C5FA89FC43FB231D3BF>]>>
startxref
59350
%%EOF


==> ut-reachability-membership.tex <==
%!TEX root = main.tex
\section{Results} \label{sec-results}
\input{subsection-vector-reachability}
\input{subsection-membership}
